Calliope-Net: Automatic Generation of Graph Data Facts via Annotated Node-link Diagrams

Graph or network data are widely studied in both data mining and visualization communities to review the relationship among different entities and groups. The data facts derived from graph visual analysis are important to help understand the social structures of complex data, especially for data journalism. However, it is challenging for data journalists to discover graph data facts and manually organize correlated facts around a meaningful topic due to the complexity of graph data and the difficulty to interpret graph narratives. Therefore, we present an automatic graph facts generation system, Calliope-Net, which consists of a fact discovery module, a fact organization module, and a visualization module. It creates annotated node-link diagrams with facts automatically discovered and organized from network data. A novel layout algorithm is designed to present meaningful and visually appealing annotated graphs. We evaluate the proposed system with two case studies and an in-lab user study. The results show that Calliope-Net can benefit users in discovering and understanding graph data facts with visually pleasing annotated visualizations.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/00-abstract.tex <==
\begin{abstract}
Graph or network data are widely studied in both data mining and visualization communities to review the relationship among different entities and groups. The data facts derived from graph visual analysis are important to help understand the social structures of complex data, especially for data journalism. However, it is challenging for data journalists to discover graph facts and manually organize correlated facts around a meaningful topic due to the complexity of graph data and the difficulty to interpret graph narratives. Therefore, we present an automatic graph data facts generation system, Calliope-Net, which consists of a fact discovery module, a fact organization module, and a visualization module. It creates annotated node-link diagrams with facts automatically discovered and organized from network data. A novel layout algorithm is designed to present meaningful and visually appealing annotated graphs. We evaluate the proposed system with two case studies with real-world datasets by domain experts and an in-lab user study. Results show that Calliope-Net can benefit users in discovering and understanding graph data facts with visually pleasing annotated visualizations.
\end{abstract}




==> sections/del-05-story.tex <==
%\section{Fact Selection and Organization}
%\rv{explanatory process completion: story -> fact organization}

%To generate a cohesive story with stronger comprehensibility (\textbf{G3}), \name develops the story based on a topic-evidence-explanation structure proposed by Kosara \etal~\cite{kosara2013storytelling}. The story starts with a topic claim followed by a series of evidence facts which are further elaborated by explanation facts. Such a structure guarantees an inverted pyramid structure that can guide the readers to the most important information in the narrative, which is often applied in data journalism \cite{hart2021storycraft} as well as visual storytelling~\cite{knaflic2015storytelling}. Also, the topic-centric structure allows the development around the topic addressing the topicality of the story. 


 %Also, the topic-centric structure allows the development around the topic addressing the topicality of the story. 


\subsection{Topic Structure}
\name organizes the facts by a tree structure where nodes represent graph data facts and links represent the sequential relations between the two facts. In the \textit{topic selection} stage, a central fact reflecting the topic is chosen as the root of the tree to emphasize the story topic. To determine the qualified facts in the latter two stages, \name characterizes the fact relations by the narrative logic and topological connections. %Below, we first analyze the advantages of the tree structure over the common sequential structure in network narratives. Then we describe the two topological and logical properties of the graph data fact relations before summarizing our story model.

%\textbf{\textit{Story Tree}} is applied due to three major concerns. First, the tree structure can represent the hierarchical nature of the selected facts, where several mutual-focus facts are combined and presented together. Second, the tree structure preserves stronger topicality as the leaf facts can be linked with the central fact by a smaller distance. Third, the tree structure enriches the search candidates in each iteration, in that one candidate fact can relate to multiple facts and each of them can generate a unique story.

%\textbf{\textit{Relations}} among the extracted facts are based on both topological and logical considerations. The topological relation is specially designed for network narratives, such as the facts sharing the same focus and the facts with the connected focuses. For example, there are plenty of visual stories in data journalism exploring the neighboring nodes of a single node \cite{2016election, proxy}. Transitions between the facts based on the logical relations contribute to the effective story delivery. Thus, we borrow the logical relations to present cohesion between graph data facts, including \textit{Similarity}, \textit{Contrast}, \textit{Elaboration}, and \textit{Generalization}. The four types of logical relations are summarized from transition taxonomy conducted by Hullman \etal\cite{hullman2013deeper} where \textit{Temporal}, \textit{Spatial} and \textit{Casual} transitions are excluded because they are not popular in static network.

In \name, the \textit{Similarity} between the facts is identified when only the measure is modified and the focus components are consistent across them. Inversely, the \textit{Contrast} relation is denoted by the deviation of the focus components when a measure changes.
\textit{Elaboration} happens when the successor fact adds more details and elaborate on the predecessor fact. \name allows three types of elaboration between the facts, (1) from a global network to a subgraph (2) from a community-level to node-level facts, (3) from an \textit{Extreme} or \textit{Rank} type of fact to a \textit{Proportion} type of fact since the \textit{Proportion} fact describes the proportion of the largest data item, which is also the focus component of the \textit{Extreme} and \textit{Rank} facts. 
\textit{Generalization} happens when the successor fact generalizes the information of the predecessor fact. \name also allows three types of generalization between the facts, which is the reverse sequence of \textit{Elaboration}.
Therefore, \name defines a relation as follows:
$$
r := \{f_p, f_s, r_l, r_t \}
$$
where $f_p$ is the predecessor fact and $f_s$ is successor fact, and $r_l$ and $r_t$ are the logical and topological relations respectively.


\subsection{Topic Selection and Skeleton Formation} \label{sec:graphtopics}

To elaborate the common topics for static networks, \name initializes the evidence skeleton based on the templates with configurable parameters. Following the specified topic, the templates can be transformed into the evidence skeleton and steer the story development in the \textit{narrative expansion} stage. The candidates are selected and evaluated based on the topic skeleton.

\textbf{\textit{Exploring Local Neighbors}} depicts one influential node with its neighborhood (e.g., \cite{proxy}). \name initializes the skeleton by selecting a central node and its neighboring facts according to the topological relations of their focus components. The template has only one parameter, indicating how the central node is identified. \name extracts the extreme fact with the specified measure and identifies the focus node as the central node of the story. Then \name identifies the topologically related facts of the central node to form the story skeleton, which elaborates the neighborhood of the single node.

\textbf{\textit{Detecting Key Players}} explores the key nodes in the network based on the topological features and node attributes (e.g., \cite{bushmoney, socialpark}). \name includes two different templates for this topic, namely, \textit{Within-Measure} and \textit{Within-Subgraph} key players.
For \textit{Within-Measure} key players, the algorithm identifies the extreme facts who have a mutual measure specified by a parameter in different subgraphs.
For \textit{Within-Subgraph} key players, the algorithm enumerates all the available measures and finds different extreme facts with different measures in a mutual subgraph. The subgraph is produced by a parameter accepting the subgraph filters (e.g., all the nodes having a categorical attribute).

\textbf{\textit{Alliance and Opposition}} analyzes the dense communications inside the communities \cite{watts1998collective} and the absence of the communications between the communities in the network (e.g., \cite{london-riots, ttip}). 
\name describes the communities divided by a topological partition algorithm. Thus it is able to reflect the intra-community alliance relationship and the inter-community opposition relationship. 
Since different partition algorithms can lead to different stories, the algorithm is one of the parameters, where the other parameter is the topological feature used to specify the central communities.
\name specifies the central communities measured by a topological feature through a \textit{Rank} fact since it is not feasible to present all communities in a single narrative due to the layout and readability concerns. The facts about other interesting communities can still be added to the story in the \textit{story expansion} stage.
    
\textbf{\textit{Revealing Hidden Ties}} identifies the weak ties between two communities whose nodes are strongly tied internally (e.g., \cite{chris}). The two communities are selected from the communities partitioned by the categorical attributes or the graph partition algorithms appointed by a parameter.
Then \name identifies the tying node which delivers an \textit{Extreme} fact measured by a topological feature in the subgraph of the two communities and connects them. Finally, \name build the skeleton with the facts about the corresponding communities as the readers are usually interested in the details of the communities.

Story generation starts by selecting the most promising topic among all the possible topics. 
It is time-consuming to enumerate all potential topics and then select the optimal one. 
Thus, \name implements a bandit strategy, which explores the candidate topics as many as possible and then chooses the most promising one. In the exploration process, the algorithm runs a randomness-based search to approximate the objective function result and calculate the result expectations of different topics. The method reduces the computation cost by approximating the objective function and using a partial candidate set. 
Assigning more trial times on the promising topics in the exploration stage can save time from exploring the unimportant topics and enlarge the chance of choosing the best one. 
The algorithm chooses the next topic to explore based on the result expectations and the topics' current trial times. The lower trial time indicates that the topic has been insufficiently explored and deserves a higher trial possibility in the following exploration.
% The algorithm tends to explore the topic with higher reward expectation and lower trial time number, which indicates the topic has been insufficiently explored.
% Since different topics may generate stories with different fact selection and organization, 
% It is time-consuming to enumerate all potential topic and then select the optimal one. 

% Thus, \name introduces a approximation-based exploration method to predict the story topic of a story before choosing the most best one. 
% There is a trade-off between choosing a more promising topic and generating a better story of one topic. 
% Balancing the trials on the different topics and 


% It is also 
% The main idea of bandit strategy is to assign more trial times on the more promising topics in the exploration process.
% The main idea of bandit strategy is to select the most promising topic to explore a time threshold and then choose the most promising one. 
% The algorithm inputs a set of topic candidates and output the most promising one among them. The algorithm starts by exploring every candidate once and initializing the reward expectations as well as the candidate test times.
% Then, t
% After finish the iterations, the algorithm chooses the most promising topic based on the average expectations. 
% In the exploration process, the algorithm will run a randomness-based search to approximate he rewards of the final story tree. The method reduces the computation cost significantly by introducing randomness and controlling the size of the candidate set. 

\subsection{Narration Expansion}
This stage iteratively runs until no facts can be added to increase the objective function. The algorithm receives a topic skeleton and adds suitable facts to it to enrich the narrative. 
The algorithm starts by initializing the candidate set, which comprises all relations the facts in the story skeleton can have.
% facts topologically or logically related to the facts in the story skeleton, with their relation instances.
The candidate set is made up by the relations rather than the facts, because the topic tree is composed by both the fact nodes and relation links. 
% TODO: 这个例子和上面的有关系的么
% Resolved by modifying the example
For example, a fact can produce multiple candidate relations as it can be related with different facts in the narrative.
% be related to multiple facts in the story tree and all the relations should be evaluated individually.
% For example, a fact can be related to multiple facts in the story tree and all the relations should be evaluated individually.
% the candidate set will all the relations. 
% TODO: based on the fact relations 这是什么，当前的？
% Resolved
In each iteration, the algorithm finds the best-fit candidate relation with the largest objective function value and add it to the structure. After that the algorithm will update the candidate set based on the fact relations. The algorithm stops and outputs the story tree when there is no more fact possible to increase the objective function value of the story tree.
% Resolved
% In each iteration, The algorithm enumerates the candidate set, which comprises all of the related facts of current story tree and add the best one to the story tree. 
% \name evaluates the story tree by the story rewards and the cost of connecting all the facts.
% TODO：这里的reward和5.2中的reward是一个么
% Add reward define in the beginning
The objective function is calculated based on the rewards valuing the selected facts and costs evaluating the relations.
The rewards comprise of three components addressing three different aspects, namely, \textit{fact scores}, \textit{story diversity} and \textit{network integrity}. 

\textbf{\textit{Fact Score}} reflects the meaningfulness of the selected facts, which is formulated as follow:
\begin{equation}
F(S) = \Sigma_{f_i \in F_S} score(f_i)
\end{equation}
where $F_S$ refers to the fact set of the story $S$ and $score(f_i)$ is calculated by Formula~\ref{eq:score}. The higher score indicates that the story comprises more facts with interesting patterns.

\textbf{\textit{Story Diversity}} estimates the diversity of fact types about a focus component. As fact scores are calculated based on type-specific functions, diversity reward can partially reduce the bias caused by the different fact types. Besides, richer diversity of the facts of a component (conditional) can elaborate the component more generally and interestingly.
The diversity reward is given by:
% Conditional diversity avoids the story being dominated by some important communities or nodes who can reach the maximum in different attributes according to Power Rule.
\begin{equation}
D(S) = - \Sigma_{focus \in FC_S, type \in T} \text{ } p(focus,type) \times ln\frac{p(focus,type)}{p(focus)}
\end{equation}
where $FC_S$ refers to the focus component set of the story $S$ and $T$ includes all the fact types described in Section 4.
% A focus component $focus$ can be either a focus node or a focus community. 
$p(focus, type)$ calculates the probability of the occurrence of the $focus$ component and type while $p(focus)$ calculates the focus component $focus$'s probability.

\textbf{\textit{Network Integrity}} measures the network coverage of the selected facts given by:
\begin{equation}
I(S) = \frac{|\bigcup V_S|}{|V|}
\end{equation}
where $V_S$ refers to the focus nodes of all the facts in the story $S$. A story with a higher integrity score can cover more nodes and represent more general network patterns.

After specifying the rewards evaluating the selected facts, we propose two cost functions to evaluate the relations of the facts.
\textbf{\textit{Cost Functions}} correspond to the two relation types we set previously. 
The cost for logical relations is calculated based on the transition probability proposed by Shi \etal~\cite{shi2020calliope} as follows:
\begin{equation}
NC(r) =  \frac{1}{ 1 + p(r)}
\end{equation}
where $p(r)$ is the probability that the relation $r$ has. 
We represent the cost by the inverse of the likelihoods' harmonic average in order to normalize the probability distribution and prevent the result dominated by some overlarge items.

Then, the topological cost of a relation is given by:
\begin{equation}
TC(r) = \begin{cases}
      0 & \text{if } r.f_s.focus \text{ is same with } r.f_p.focus\\
      1 & \text{if } r.f_s.focus \text{ is connected with }  r.f_p.focus\\
      \infty & \text{if }  r.f_s.focus \text{ is not connected with } r.f_p.focus\\
    \end{cases}       
\end{equation}
where $r$ is the relation. Facts related topologically (e.g., within the same node, with a connected edge) can relieve readers' burdens and promote readability. 
After obtaining the two costs separately, we formulate the overall cost by:
\begin{equation}
C(r) = \frac{\gamma_1 + \gamma_2}{\frac{\gamma_1}{TC(r)} + \frac{\gamma_2}{NC(r)}}
\end{equation}
We represent the cost by the harmonic mean of the two costs weights $\gamma_1, \gamma_2$ to prevent cost calculation being dominated by the bigger cost. Besides, the harmonic mean can also resolve the issues of the infinite topological cost caused by the facts without any topological connection. 


\subsection{Text Generation} \label{sec:textgeneration}
\name includes a text summary of the graph story and a series of annotations for the accompanying facts. To generate comprehensible text annotations (\textbf{G2}), we involved the graph mining experts in our development phase and employ a template-based text generation method. 
The experts created a set of annotation examples for the different types of facts. After transforming those annotations into the templates, we also invited the experts to read the generated text and further fine-tune them. We design various templates for different types of facts, with the empty slots filled by partition methods, measures and focus subjects. 

To improve the readability of the text annotations, we introduce measure translation and conjunctions (e.g., similarity, to elaborate) in the templates. The graph data facts comprises a series of topological measures such as density, triangle participation rate (TPR). Those will cause extra burdens for the readers without network background. Thus, we describe them in a more understandable way, while preserving the original terms in the annotations. For example, density, inside edge number and TPR all reflect the internal cohesion of a community in the network. 
The templates include a slot called \{Measure Translation\} which can be filled by the converted measure description as the appendix shows. 
For instance, if a community reaches the extreme of TPR, \name will describe it as \textit{The community is a cohesive community based on the highest triangle participation rate.}
Experts agree that though the measure translation is not rigorously stated, the enhanced comprehensibility outweighs the drawbacks.
In the text summary, using conjunctions can imply the relationship between two successive sentences and improve the fluency of the text. We generate the conjunctions based on the narrative relations such as the \textit{Similarity} of the facts. The detailed templates can be found in the appendix.


%%-----------------------------------------------------------
%archive
%so that the facts linked with previous facts can also be touched when only the facts directly linked with the last searched fact can be added in the sequential model. --?
%TODO: 这句话补充完，或者你写一下这句话的中文，how/why it increases the diversity
% Resolved, one candidate fact can produce multiple relation candidates

%The tree structure has three main advantages over the sequential models used in Calliope. Firstly, the tree structure meets the presentation structure and represents the hierarchical nature of the annotated network, where several mutual-focus annotations are combined and presented together. Secondly, the tree structure preserves stronger topicality by allowing multiple facts directly linked with the central fact. For example, for a story exploring the neighborhood of a central node, the tree structure allows the facts focusing on the neighboring nodes directly added to the fact of the central node, while the sequential structure only allows one fact connected with the center. Furthermore, the tree structure enhances the diversity of the search candidates in each iteration in that, the facts linked with previous facts can also be touched when only the facts directly linked with the last searched fact can be added in the sequential model.

%which guarantees the hierarchical and sequential structure of the network annotations. 
% Thus, we can represent a story by:
% $$
% S:= \{root, facts, relations\}
% $$

% 
%TODO: add a short description of the relation between STORY TREE and FACT RELATION, why story structure includes the two key components/consider the two aspects. Story Tree constructs the skeleton of a story, Fact Relations joint the skeleton.
% Resolved
% Add description behind it. 
% Goal: story with a proper structure and sequence. structure->tree, sequence->relation. The structure contains the relations

% Tree is a data structure when the relation and fact correspond to the links and nodes respectively.



%namely, Global-Subspace, Community-Node and Proportion elaboration. Global-Subspace elaboration means that the successor fact's subspace changes from global network to a subspace when other fields follow the successor fact. Community-Node elaboration means that the successor fact is partitioned by certain attribute when the predecessor fact has no partition field. Proportion elaboration means that the successor fact is of proportion type when the predecessor fact, whose other fields are same with the successor, is an extreme or rank. It is inspired by the notion that the proportion fact only describes the extreme item's proportion.

%\begin{itemize}
    %\item \textit{Similarity} indicates that two ensuing facts presents sort of similarities in the fact data. Thus, \name uses the statistical similarity of the fact data and focus subjects when a breakdown changes.
    %\item \textit{Contrast} indicates the two ensuing facts contrast with each other. Thus, \name uses the statistical deviation of the fact data and focus subjects when a breakdown changes.
    %\item \textit{Elaboration} happens when the successor fact adds more details and elaborate on the predecessor fact. \name allows three types of elaboration between the facts, namely, Global-Subspace, Community-Node and Proportion elaboration. Global-Subspace elaboration means that the successor fact's subspace changes from global network to a subspace when other fields follow the successor fact. Community-Node elaboration means that the successor fact is partitioned by certain attribute when the predecessor fact has no partition field. Proportion elaboration means that the successor fact is of proportion type when the predecessor fact, whose other fields are same with the successor, is an extreme or rank. It is inspired by the notion that the proportion fact only describes the extreme item's proportion.
    
    %\item \textit{Generalization} happens when the successor fact generalizes the information of the predecessor fact. \name allows three types of generalization between the facts, namely, Subspace-Global, Node-Community and Proportion-Followed generalization. Subspace-Global generalization means that the successor fact's subspace changes from a sub-network to the global network when other fields follow the successor fact. Node-Community generalization means that the predecessor fact is partitioned by certain attribute when the successor fact has no partition field. Proportion-Followed generalization describes the means that a proportion fact fact is by an extreme or rank fact, of which other fields remain same.
%\end{itemize}

%
%\subsection{Search Framework}

%The search process will take input of the built evidence skeleton and produce a complete story by adding the most suitable facts. The algorithm has following three phases.
%\begin{itemize}
    %\item \textbf{Stage 1: Topic Selection} The algorithm starts by selecting the most promising topic among the all possible topics. There is a trade-off between choosing a more promising topic and generating a better story of one topic. Thus, we implement a Bandit strategy to balance the time spent on the exploring topics and exploiting the most promising topic. 
    %\item \textbf{Stage 2: Initialization} The algorithm then works by generating the tree skeleton based on the selected topic. In this way, \name can ensure the topicality of the generated story by rendering the consequent fact search process guided by the topic.
    %\item \textbf{Stage 3: Story Expansion} In this stage, the algorithm runs iteratively to find the best-fit fact link and update the candidate set. To control the story length, Calliope sets an early stop mechanism to stop the story expansion when the fact number hits the upper constraint.
%\end{itemize}


%The algorithm starts by selecting the most promising topic among the all possible topics. There is a trade-off between choosing a more promising topic and generating a better story of one topic. Thus, we implement a Bandit strategy to balance the time spent on the exploring topics and exploiting the most promising topic. 
%In \name, a topic is with a specific topic type and some configurable parameters. 
%The above four topics along with a topic inclusively for dynamic network, \textit{Exploring the Evolution of Associations Over Time} are summarized in the narrating network study conducted by Bounegru \etal \name excludes \textit{Exploring the Evolution of Associations Over Time} as dynamic network has not been supported yet. 

% As there can several communities partitioned and
    % As a result, the partition algorithm is one of the parameter in the template and the other one is the initial community measure. TO avoid introducing extra fact, \name uses the rank fact as the topic fact and then searched the top facts about the communities. The rank fact embraces the top-3 communities measured by a topological feature e.g. separability, which can be the most interesting alliances. 
    % It is noted that the measure is only used in constructing the topic and other measures can also be employed in the evidence and explanation.
    
% The topic explores two separate communities in a network. \name first find two separable communities with the related facts about the two communities.  Stories with the topic build their skeletons by detecting all the facts about the selected communities. To avoid spending unnecessary time on the vast number of unpromising topics, the algorithm filter out the communities with lower separability or few interesting facts. 

% Like \textit{Alliance and Opposition}, \name need to find two separable communities. But the focus of the topic will be the node connecting the two communities, which means the node has highest degree within the two communities. Stories with the topic start with a extreme-degree fact in a subspace constructed by two selected communities. Then, the algorithm elaborates on the topic by adding the facts about the two communities.

%TODO: ADD some variable definition (e.g., what is T, \hat{x}, etc.)
% Resolved

% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% If we put the algorithm here:
% The algorithm starts by selecting the most promising topic among all the possible topics. Since different topics may generate stories with different fact selection and organization, it is time-consuming to first enumerate all potential topics and then select the optimal one. There is a trade-off between choosing a more promising topic and generating a better story of one topic. %Thus, we design a bandit strategy, which explores different topics with a time threshold before exploiting the most promising topic.
% Thus, \name implements a bandit strategy to select the best-fit topic. The main idea of bandit strategy is to explore the candidate topics as many as possible and then choose the most promising one. 
% As Algorithm-\ref{algo:topic} shows, the algorithm inputs a set of topic candidates and output the most promising one among them. The algorithm starts by exploring every candidate once and initializing the reward expectations $\hat{x}$ as well as the candidate test times $T$.
% Then, the algorithm runs iteratively by exploring the most promising topic, which is chosen based on a score, i.e. $scores[i]$ calculated by the topic test time $T[i]$, topic reward expectation $\hat{x}$ and the total test time $T_{all}$ until a test time limit is hit. After finish the iterations, the algorithm chooses the most promising topic based on the average expectations. 

% If we put the algorithm in the appendix




% \name initializes by enumerating all the possible topics and exploring each of them once. Then \name selects the next topic to explore based on the following criteria:
% $$
% value = \hat{rewards}_t(m) + \sqrt{\frac{ln m}{T_{t,m}}}
% $$
% where $m$ is the test number, $T_{t,m}$ is the test number of the topic $t$ and $\hat{Rewards}_t(m)$ is the average reward. \name selects the topic with highest value and explore it. The higher the average reward is, and the lower number of test is, the more likely the topic will be test.


% Since the algorithm is closely related to the story expansion, we will describe the details of the algorithm in the Story Expansion section. 
% \name incorporates a similar simulation approach used in Monte-Carlo Tree search in the exploration process, in which, \name selects the next fact randomly in the candidate set and calculates the final rewards. After each exploration, \name will update the values based on the exploration result.

% \begin{algorithm}[]
% \SetAlgoLined
% \KwIn{Topic candidate list, $topics$}
% \KwOut{Best Topic, $topic_best$}
%  \While{$T_{all} < limit$}{
%     $values = zeros(len(topics))$\;
%     \For{\texttt{$i:=0, i < len(topics), i++ $}}{
%         $values[i] = \hat{x}[i] + \sqrt{\frac{lnT_{all}}{T[i]}}$ \;
%       }
%       \EndFor
    
%     $best := argmax(values)$ \;
%     $topic := topics[best]$ \;
%     $score := explore(topic)$ \;
%     $\hat{x}[best] = \frac{\hat{rewards}[best] * T[best] + score}{T[best] + 1}$ \;
%     $T[best] = T[best] + 1$ \;
    
%  }
% %  $values = zeros(len(topics))$\;
%     % \For{\texttt{$i:=0, i < len(topics), i++ $}}{
%     %     $values[i] = \hat{rewards}[i] + \sqrt{\frac{lnT_{all}}{T[i]}}$ \;
%     %   }
%     %   \EndFor
    
%  $best := argmax(\hat{x})$ \;
%  $topic_{best} = topics[best]$
%  \caption{Topic Selection} 
%  \label{algo:topic}
% \end{algorithm}



% \subsection{Initialization}
% After selecting a topic, \name initialize the story skeleton and candidate sets by rule-based approaches. 

% The story skeleton includes facts that directly or indirectly elaborates the selected topic.
% The rules for the different topics are followed:

% \begin{itemize}
%     \item \textbf{\textit{Exploring Local Neighbors}} 
%     \item \textbf{\textit{Detecting Key Players}} 
%     % As there are two types of configs about the topic, the initialization process also employs two distinct ways. For \textit{Within-Measure} key players, the algorithm detects divides the nodes into different communities and find all the extreme facts of one single measure together with the extreme fact in the global network. For \textit{Within-Subspace} key players, the algorithm enumerates all the available attributes of nodes and find different extreme facts measured by different attributes.

%     \item \textbf{\textit{Alliance and Opposition}}

%     \item \textbf{\textit{Revealing Hidden Ties}} 

% \end{itemize}


% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% If we put the algorithm here:
% This stage runs iteratively until there is no fact can be added to gain more rewards against the additional cost. As Algorithm \ref{algo:expansion} shows, the algorithm inputs a story skeleton $S$ and add the suitable facts to it to form a complete story. 
% The algorithm starts by searching all the candidate relations of the initial skeleton. The valid candidates include all the facts which are related to the facts already in the current story tree in terms of the logical relation or topological relation mentioned before.
% In each iteration, the algorithm search the best-fit candidate relation $r_{next}$ which has the largest rewards and add it to the story tree by $addLink$ function. After that the algorithm will update the candidate set based on the fact relations. The algorithm stops and outputs the story tree when there is no more fact possible to benefit the evaluation of the story tree.


% If we put the algorithm in the appendix:


% After the process, the algorithm will update the candidate set by removing all links involving the newly-added fact and adding the relations possible to be connected with the newly-added fact. 
% Different from Calliope, \name's candidate is a relation instance rather than a fact in that the benefit of adding a fact to the story tree varies according to where it is added. 
% \name determines the relation between two facts based their narrative transition and topological connections. 
% A relation $r$ should meet the following two conditions if it is a candidate of the story $S$:
% $$
%     r.f_p \in S.facts \text{ and } r.f_s \not\in S.facts
% $$
% where $S.facts$ is the fact set of the story $S$ as well as $r.f_p$ and $r.f_s$ are the predecessor and successor facts of the relation $r$ respectively. The first condition requires that the relation should be added to one of the fact within the story tree. Thus it ensures every possible relation is either logical or topological in the final story. In addition, the second condition requires that there is no loop in the tree structure and prevents the story falling into circular narrative. Even though circular narrative is a common style in storytelling, it can lessen the story length and is not common in network narratives.



%TODO: 这部分可能放到对应的formula描述里：
% Resolved, put the content in the previous story expansion subsection.
%After specifying the rewards and costs, we can calculate a story score by adding them up with proper coefficients. The detailed formulas of the reward and cost functions can be found in the appendix. 




% For each candidate relation, the algorithm calculates the rewards and cost of adding the relation to the current story. Then the algorithm calculates a beneficial score as follows to decide which relation is most beneficial for the current score:
% $$
% \delta g = \frac{rewards(S')-rewards(S)}{cost(r)} 
% $$
% where $S'$ is the story tree formed by adding relation $r$ to the current story tree $S$. The score reflects the extent to which the information that the audience can gain from the new story within a reading cost.

% As the previous topic selection section mentions, the topic exploration also involves with the search process. \name ease the computation burden by introducing a randomness search strategy in the story expansion. The algorithm only enumerates a partial candidate set in the exploration process. The algorithm chooses the partial set based on a Exponential distribution of the fact's story-blind cost score as follows:
% $$
% c = \frac{r.cost}{f_s.score}
% $$
% $$
% p(c) = \mu \lambda e^{-\lambda c}
% $$
% The story-blind cost score approximates the potential cost against of the benefits of adding the relation. The distribution enhances the possibility of relation with higher score and lower cost being enumerated. The parameter $\mu$ plays a role of scaling factor and is able to control the size of the candidate set.
% \begin{algorithm}[]
% \SetAlgoLined
% \KwIn {Story Skeleton $S$}\\
% \KwOut{ Complete Story, $S$}
%  $candidates = initializeCandidates(S)$\;
%  \While{True}{
%     $g_{max}$ := 0\;
%     $r_{next} := null$\;
%       \For{\texttt{r in candidates}}{
%         $S' := addLink(S, r)$ \\
%         $g = rewards(S') - rewards(S)$ \\
%          \If{ $g > g_{max}$}{
%               $g_{max} = g$\;
%               $r_{next} = r$\;
%           }
%       }
       
%         % \State \texttt{<do stuff>}
%       \EndFor
%       \If{ $r_{next} = null$}{
%               break\;
%       }
%     $candidates_{new} = getRelatedFacts(r_{next}.successor)$\;
%     $candidates_{new} = candidates_{new}.filter(r=>r.succssor \not\in S.facts)$\;
%     $candidates_{old} = candidates.filter(r=>r.succssor \neq r_{next}.successor)$\
%     $candidates = merge(candidates_{new}, candidates_{old})$
% %   instructions\;
% %   \eIf{condition}{
% %   instructions1\;
% %   instructions2\;
% %   }{
% %   instructions3\;
% %   }
%  }
%  \label{algo:expansion}
%  \caption{Story Expansion Algorithm}
% \end{algorithm}



% \subsection{Rewards and Cost}
% \name employs a reward function that estimates the quality of the generated story with three criteria, namely, fact interestness, diversity and integrity. The fact interestness is calculated by adding up the scores of the all facts describe in the previous section.

% \noindent
% \textbf{Diversity} estimates the conditional diversity of fact types of a focus subject. Compared to Calliope, which use the diversity of fact types within the whole story, \name applies the conditional diversity, in that the generated annotations have a hierarchical structure and the mutual-subject annotations should not be too similar.  
% $$
% D(S) = - \Sigma_{v \in S.V, f \in S.F} \text{ } p(v,type) \cdot ln\frac{p(v,type)}{p(v)}
% $$
% Here, $S.F$ and $S.N$ are respectively the fact set and subject set of the story tree.

% \noindent
% \textbf{Integrity} estimates the network coverage of the generated story.
% $$
% C(S) = \frac{\bigcup S.V}{G.V}
% $$

% The cost contains two types costs, topological cost and logical cost. 

% \noindent
% \textbf{Logical Cost}
% We borrows the statistical analysis on the logical connections of diverse fact types. The study includes the conditional possibility of the connection types after a fact type. 
% Calliope represents the logical cost as follows:
% $$
% LC(r|f) =  \frac{1}{ 1 + p(r | f)}
% $$
% Here, $p(r|f)$ is the possibility that a connection is added after the fact $f$. From the formula, we can conclude that the more possible a connection is added the fact, the bigger cost will be there.

% \noindent
% \textbf{Topological Cost}
% Calliope uses topological cost to motivate the elaboration on one focus subject as the merged annotation takes up less space and reduces the presented elements on the network. 
% $$
% TC(r|f) =      \begin{cases}
%       0 & \text{if } r.f_s.focus \text{ is same with } f.focus\\
%       1 & \text{if } r.f_s.focus \text{ is different with } f.focus\\
%     \end{cases}       
% $$
% Here $r.f_s.s$ is the subject of relation $r$'s successive fact and $f.s$ is the subject of the fact $f$. The definition means that topological cost only works when the relation and the fact have different subjects.

% Thus, the overall cost of the relation $r$ is the sum of the above two costs:
% $$
% C(r|f) = \mu_1 LC(r|f) + \mu_2 TC(r|f) 
% $$

==> sections/tmp.tex <==
% Narrative visualization has captured the attention of the visualization community~\cite{kosara2013storytelling, hullman2013deeper, borkin2015beyond, lee2015more} in the past decade. 
% Recent research~\cite{hullman2013deeper, borkin2015beyond} demonstrate the benefits of narrative visualization in improving memorability and comprehension. 
% Lee \etal~\cite{lee2015more} discuss visual storytelling's creation process, incorporating steps involved in identifying findings, structuring a story, and communicating the story.
% Other researchers~\cite{stolper2016emerging, mckenna2017visual} investigate the design factors of narrative visualization.
% These theoretical studies have in turn led to the emergence of increasingly expressive interactive visual authoring tools~\cite{amini2016authoring, ren2017chartaccent, brehmer2019timeline}.
% Kosara \etal~\cite{kosara2013storytelling} emphasized annotations' effects in augmenting stories and guiding users in visual data-driven storytelling.
% Kandogan \etal~\cite{kandogan2012just} build a system to automatically annotate the clusters, outliers, and trends along with their semantic descriptions in point-based multi-dimensional visualizations. 

%Kandogan\cite{kandogan2012just} introduces the concept of instant annotation, in which a diagram is automatically annotated when a person interacts with it. Similarly, Bryan et al.\cite{bryan2016temporal} introduced a method to automatically label graphs describing time-oriented data based on visual salience and salient features in the data during interactive exploration. Richard Brath & Martin Matusiak.\cite{brath2018automated} proposed the concept of automated annotation, which is similar to natural language generation for news, where natural language stories are generated entirely from datasets. Automatic annotations provide a new focus for the audience, allowing for timely updates and delivery of visualization information. Design guidelines for annotated charts are also presented for different chart characteristics. Ren et al.\cite{ren2017chartaccent} classified annotated charts into the form of annotation (text, shapes, highlights, and images.) and the target type of annotation (data items, structural chart elements, coordinate spaces, and prior annotations).
%Tableau Desktop\footnote{Tableau Software. http://tableau.com.} offers several more basic annotation Chart options. For example, Tableau allows users to add trend lines to charts, and text annotations for markers can be data-driven, referencing the underlying data properties of the marker. ChartAccent\cite{ren2017chartaccent} is an interactive tool that allows people to generate data annotations manually, and it surpasses Tableau in many ways. Highlighting markers in chartAccent is easier and more flexible than Tableau is more straightforward and flexible, eliminating the need to create collections explicitly; selected tags can be highlighted directly without affecting unselected tags.
%Contextifier\cite{hullman2013contextifier} provides an algorithm for selecting annotations that automatically creates a stock timeline chart and matches the appropriate annotation to the line chart visualization regarding the content in the news article, thus generating a stock behavior visualization with annotations. Kori \etal~\cite{latif2021kori} analyze the design space of chart–text references through news articles and scientific papers. is a tool that automatically provides annotation suggestions using natural language, which allows for combining text and diagrams through manual interaction. It solves the problem of viewers reading diagrams and going through text annotations, which leads to distraction and cognitive load.
%two directions: automatic annotation text generation, automatic layout

The annotated visualization is one of the seven genres of narrative visualization proposed by Segel and Heer~\cite{segel2010narrative}. Annotations play an important role in various genres of visual narratives through guiding users' attention graphically and providing the data context ~\cite{kosara2013storytelling, choe2015characterizing, ren2017chartaccent}.
% In this paper, annotations are graphical overlaid information, such as graphical markers (such as arrows and trend lines) and/or text (such as data values or commentary), on top of a visualization to add contextual information regarding the data in the plot.
Ren \etal~\cite{ren2017chartaccent} propose a design space for annotated visualizations, identify the form of annotation (text, shapes, highlights, and images.) and the target type of annotation (data items, structural chart elements, coordinate spaces, and prior annotations). We exploit their design space and determine our visual encoding based on it in Section ~\ref{sec:visual}.
To create the annotations efficiently and effectively, a wide range of data-driven techniques and tools~\cite{kandogan2012just,hullman2013contextifier,bryan2016temporal,latif2021kori} have been proposed and developed for different use scenarios. Contextifier~\cite{hullman2013contextifier} targets at data visualization in news articles and implements a tool to automatically generate annotated stock line chart. They propose an annotation algorithm that involves visual salience, contextual relevance, and detection of key events in the company's history. Brian \etal~\cite{bryan2016temporal} study the annotations on the temporal layouts which enable the creation of the annotations with proper placement and interesting patterns. Instead of manual creation of annotations, Brath \etal~\cite{brath2018automated} automatically generate annotations, to ``automatically finding the most pertinent meaning in a given dataset.'' Kori \etal~\cite{latif2021kori} analyze the design space of chart–text references through news articles and scientific papers. Based on the analysis, they propose a mixed-initiative interface that enables the synthesis of text and charts through interactive references.

Though the above works enable the data-driven annotation creation, the annotation generation for the graph data have been insufficiently touched. Considering that the ability to tell stories with graph data is underestimated, Bounegru \etal~\cite{bounegru2017narrating} analyze a series of graph stories in journalism and concluded five perspectives for narrating graph stories. The five perspectives are later used as graph topics in Section \ref{sec:graphtopics}. Bach \etal~\cite{bach2016telling} discuss how to use the visual expressiveness and familiarity of comics to communicate changes in dynamic graphs. As a result, Datatoon~\cite{kim2019datatoon} is an interactive authoring tool that facilitates the creation of data comics with recommendations of four automatically-detected structural patterns including articulation points, cliques, hubs, and communities. To alleviate the barriers for telling graph stories, we provided a flexible and efficient generation and editing tool that automatically finds data facts both in attributes and structural and tells stories in the form of annotated visualizations.


---------------------------

% feedback
%According to our interviewees, data journalists in Austria have basic computer literacy as well as basic statistical knowledge. The exploration and research phase was organized depending on the journalists’ personal preferences and skills. The interviews indicated that journalists are comfortable with combining different tools such as Microsoft Excel, Google Spreadsheets for data analysis and other tools such as Evernote [eve] for storing notes, which were found during the exploration or research phase. Furthermore, the research documentation has been reported to be in both electronic and paper forms. A commonly followed standard workflow or specific user description could not be identified on the basis of the conducted interviews. Due to the investigative character of their work, the interviewed journalists have to deal with a wide range of data sources originating from various other domains. However, deadlines and lack of time (and resources) for extensive analysis are also limitations to data-intensive news work. When it comes to visualization techniques, standard business charts such as bar charts, line plots or pie charts were mentioned as being known and used. The journalists stated that they prefer easy-to-use interfaces and visualizations. The journalists reported that they usually carry out the research phase on a news story alone. The next steps of designing infographics and drafting the final article are then mostly done in teams of two to three people.
%The interviewed journalists either start from a story idea and subsequently search data to support the evidence, or they start from data and develop a story idea revolving around their findings. Before writing a story, however, they would conduct interviews because it is their journalistic responsibility to compare information from multiple sources. In this process, data analysis helps them to identify possible interview partners. One interviewee also mentioned that data-based insights help him to get more time for investigation approved.
We summarize the interview results as follows.

\underline{\textit{Tools and workflows.}} 
All the journalists reported to use different tools at different stages of data-driven news which involves graph data. The exploration and organization style and process rely largely on the journalist's personal preferences and skills. Some would work with data analysts in the data exploration stage and some would work with graphical designers at the presentation stage. However, due to tight schedule and the cost to communicate and collaborate with others, in most cases, they usually need to finish most of the data-driven exploration and creation by themselves, sometimes they leave the final design optimization to the specialist to help with the overall appearance and theme. The most frequently used tools for data exploration and presentation are gephi~\cite{bastian2009gephi} and Tableau~\cite{chabot2003tableau}. There are typically two workflows they follow when creating the graph visualization. 
One common workflow is that they have one or several potential themes in mind and then validate or enrich their assumptions with evidences found in graph visualizations.
The other is that the journalist is given some interested datasets and needs to organize a news story around the data facts in the exploration phase.


\underline{\textit{Visualization styles and formats.}} 
When discussing how to visualize the graph data, all the interviewees mentioned that they prefer to apply node-link diagrams with annotations for better understanding and flexible adjustments. 
% node-link
E4 mentioned that ``\textit{node-link diagrams are easy to understand and naturally present the relationship between nodes.}''
E3 complemented that ``\textit{node-link diagrams are more flexible for creation, i.e., highlight nodes, add annotations; visually appealing and eye-catching, which is essential for visualization in journalism.}'' 
% force-directed
E3 and E4 mentioned other graph representations and commented that, ``\textit{compared to arc diagrams, circle layout, the force-directed layout of node-link diagram is more intuitive to show the distance between nodes. It is also more inclusive, can contain a larger scale of data, and show the information tightly.}'' 
% annotation
They used annotations frequently in their creation process after exploring the graph structure and data facts to mark down important information and provide details directly to the reader. They consider it a necessary to provide text annotations so that readers get the information directly from the visualization while reading the news article. Titles and other supporting text are commonly added to the visualization to facilitate understanding. In addition, E1 concluded that ``\textit{considering the data-ink ratio, I prefer creating visualizations in a more concise way, and node-link diagrams with annotations are most suitable to provide informative graphs.}'' 
% Sometimes maps are also used, if the data includes geographical information.
% and bring more messages

% workflow and Design difficulties.
\underline{\textit{Difficulties and Suggestions.}} 
We also summarize the exploration and design difficulties they encounter when creating graph-related data news. One major difficulty is to make sense out of unfamiliar datasets in a limited time range.
E1 said that she often needs to work on several topics at the same time and doesn't have enough time to fully explore the dataset, ``\textit{in most cases, I do not have background knowledge about the dataset or topic, so I have to explore aimlessly at the beginning, analyzing the features of the data from different aspects and looking for starting points.}''
E4 agreed that ``\textit{there are quite a few situations where I have no idea how to get started. I sometimes take inspiration from other articles.}'' 
Another challenge is the time-consuming and labor-intensive operations in creating visualizations.
They often use Gephi to adjust the layout to generate the node-link diagram and then import it to vector editing tools such as Adobe Illustrator to add annotations and modify the style.
E3 complained that ``\textit{sometimes it takes me hours to simply adjust the position of the annotation mannually for a more aesthetically appealing result.}''
In addition, E2 commented that ``\textit{for me, those graph visualization tools are quite helpful, but they are not 'intelligent' enough, for example, some common functions such as node search are hidden deep in Gephi and require additional workload to search.}'' 
All the interviewees agreed that a certain level of automation would facilitate and inspire their creation. 
%The network often possess hundreds of or even more nodes and it is difficult for users to extract the effective facts from the data in a short time. 
E1 said that ``\textit{automated fact discovery and organization will help me get familiar with the data and find the narrative perspective more quickly.}''
E2 complemented that ``\textit{I need a quick preview of what the visualization will look like and try out different outcomes.}''
E3 emphasized that ``\textit{insight suggestion would be useful but the premise is that the algorithm is reliable.}''
While those journalist who create data-driven news articles are open-minded and interested to apply state-of-art technologies or apply advanced tools, they believe that the level of interaction is also very important in daily practice.
For example, E1 mentioned that ``\textit{the patterns identified in the data are sometimes superficial and require additional information to explain.}''%domain knowledge for deeper insight
Therefore, convenient editing is necessary. %provide rich interaction
E3 said that the current softwares could help the creation process at different stages but ``\textit{the one-stop creation platform is always preferred, so that I could edit all the materials more efficiently. }'' %import data, suggesting insights, refining content, adjusting extra information such as text, layout, style, etc.
E2 mentioned that ``\textit{compared with heavy and complex softwares, I prefer a concise interface with a simple toolbar and real-time display.}'' %gephi complexity

% 需求 需要这个工作
% 哪些方式需要自动化
% 哪些需要编辑
% 自动化 + 手工自定义
% TODO：会不会有在诱导的感觉
%\underline{\textit{Interactions.}}
%time-consuming, improve efficiency: fact discovery, POC network structure - different layout for explanation/presentation effectively and aesthetically
%automatic approach - 



% \subsection{Preliminary Analysis}
% To specify the design requirements, we conducted a preliminary analysis through a series of expert interviews and a literature survey.
% TODO: 如果没有合适的表格，需要多加几个reference 
% 从下到上三个角度讲 %
% venturini201711: building blocks of the story: data facts
% bounegru: structure of the story: topics;
% venturini2017visual: layout and presentation

% \rv{expert interview with 4 data journalists - determine to use 1.annotation 2.node-link diagram 3.topic-driven(explo}

% We ran iterative interviews with two experts in network analysis during the entire development. They are both experienced network researchers in the computer science department of a top university. We also collected and analyzed the papers about the properties, organization and presentation of network narratives to extract the requirements of building a successful network story. 
% Venturini \etal \cite{venturini201711} analyze the visual properties affording the narration in networks (e.g., topology, density of connections), which become the fundamentals of our data fact designs. 
% The narrative building blocks, data facts are organized based on four particular structures, which are extracted from the study conducted by Bounegru \etal \cite{bounegru2017narrating} in which they summarize five types of network narratives.
% For the presentation of network stories, Venturini \etal \cite{venturini2017visual} emphasize that using position, size and hue encoding can guide users in the interpretation of network topology effectively, supporting our story presentation.
% After summarizing the feedback from experts and the knowledge derived from the literature review, we conclude three key aspects of facts regarding to visual storytelling for networks.

% \noindent
% % TODO: 补充一个具体的Data fact的example, 再说we introduce the official definition in section 4.1.
% % Resolved: Stem CELL wars %
% \textbf{I1. Data Facts.} Data facts are introduced as building blocks to formulate visual data stories~\cite{lee2015more}. Previous work applied the automatic fact extraction methods for multi-dimensional data and formulate a similar definition as a 5-tuple~\cite{wang2019datashot, shi2020calliope}. For example, in a graph visualization analyzing the citations in stem cell science \cite{stemcellwars}, the fact presenting the author node with the highest connections in the graph can be regarded as an extreme fact partitioned by node and measured by degree. 
% The common data fact types, for example, extreme, rank, are also observed in network narratives. Compared to the spreadsheet, the graph stories rely on the effective delivery of the topological structure. The experts acknowledged that it is necessary to introduce the topological partition and measures in the graph data fact formation. %Based on the insight, we define the fact by a 5-tuple and introduce its precise definition in Section 4.1.

% \noindent
% % TODO: why we need annotation再加一句在expert confirm之前(without annotation, xxx) 这里可以加1、2个references
% % Add literature on annotations' importance 
% % Add a real example
% \textbf{I2. Annotations for Graph Storytelling.} Since graph visualizations are often presented as node-link diagrams, annotation on the existing diagram is a natural and most used narrative genre for graph storytelling. Annotations play an important role in narrative visualization by revealing key points and explaining the context \cite{bounegru2017narrating,ren2017chartaccent}, and are applied in data journalism. For example, in a graph story from \textit{New York Times}%\textit{``Chris Christie and the Lane Closings: A Spectator's Guide''} 
% \cite{chris}, the editors use text annotations to elaborate the nodes representing the staff related to Chris Christie in New Jersey.
% The experts confirmed the applicability of annotated charts to reveal graph stories as they are accessible and easy to read for a more general audience through various media, such as newspapers, posters and websites. 
    
% \noindent 
% %TODO: why we need narratives, explicitly claim (to communicate, why we need stories, without stories/topics/themes, xxx) %%
% \textbf{I3. Narrative Topics.} Stories usually revolve around specific topics, and graph stories are no exception. Kosara \etal claim that besides the information delivery, it is also important to raise the readers' awareness and interest in a specific topic \cite{kosara2013storytelling}. The absence of an explicit topic in the story can lead to a loosely structured story and disturbs the readers. Thus, it is important to develop the story with a clear and appropriate topic. Bounegru \etal \cite{bounegru2017narrating} summarize five typical topics from the collected narratives, namely, \textit{Around Single}, \textit{Key Players}, \textit{Alliance and Opposition}, \textit{Reveal Hidden Ties}, and \textit{Exploring the Evolution of Associations Over Time}. Since we do not consider dynamic networks at the current stage, the last topic is not included. Our experts confirmed that the four topics are reasonable as they satisfy the needs of analyzing the topological patterns of a static network.


----------
\subsection {Design Goals}
Based on the above analysis, five design goals are proposed.

\noindent
% \textbf{G1. Extract meaningful facts about a network automatically.} 
%TODO: 加一下the need for automatic extraction (save time/efforts/pre-knowledge, etc.) 
% network data is complex
% extracting facts needs network knowledge
\textbf{G1. Extract meaningful and interesting graph data facts.} 
Graph data facts, which are statistical information extracted from the network, are the building blocks of an annotated chart. Extracting meaningful data facts is also a challenging task due to the complexity of the data and the abstractness of the fact model. To ensure the quality of result, it is necessary to make sure that the facts extracted are credible and interesting.
%Besides, the lack of the network knowledge also creates extra burden for users to choose the suitable facts.
% It is necessary to use an automatic extraction algorithm for the facts.
% Extracting meaningful facts requires a rational fact model and appropriate quality evaluation.
% Thus, it is necessary to use a rational fact model and appropriate quality evaluation to ensure the meaningfulness of the extracted facts. 
% While the graph data facts share similar structure and types with the facts from multi-dimensional data, they still differ due to the topological features and graph partitions. 
% Thus, an adaption is required to integrate the topological features and graph partition algorithms.
% into the fact formalization and evaluation process. 
% Extracting data facts is also a challenging task for non-expert users due to the complexity of the data and the abstractness of the fact model. %Besides, the lack of the network knowledge also creates extra burden for users to choose the suitable facts.
% Hence, it is necessary to use an automatic extraction algorithm for the facts.
% The network often possess hundreds of or even more nodes and it is difficult for users to extract the effective facts from the data in a short time. 
% Besides, the fact formation is closely related to the knowledge in network analysis, which is lacked by most of the non-expert users. Thus it is infeasible for users to extract the network facts manually and necessary to use an automatic algorithm.

\noindent
\textbf{G2. Organize facts into meaningful topics.}
An appropriate topic is essential to attract readers' attention and increase their memorability~\cite{kosara2013storytelling}. Common narrative topics around networks usually derive from a set of key nodes or groups and their association with each other~\cite{bounegru2017narrating}. The organization of meaningful topics should be considered in the graph fact selection process.

% fact organization
%Categorize and organize data facts into certain topics with a proper narrative flow for better understanding
% Collecting the generated data facts and transforming them into a comprehensible story involves many factors. 
% Among them, the structure and sequence contribute most to the understanding of a story~\cite{lee2015more} since they can improve the cohesion and logic of the story.
%Kosara summarized an CFO structure for data stories and divide a story into four components namely, claim, evidence, explanation and conclusion~\cite{}. %Among the four components in the narrative structure, claim or topic is the beginning of the story which guides the latter story pieces. 
%Narrative topics based on graph data usually derives . There are different network properties


%It is required to extract or summarize common topics of graph data from previous literature~\cite{bounegru2017narrating}.
% and existing cases in data journalism.



% Moreover, since the sequence of the data facts determines the cohesion of the story, the logical connections between the data facts should be established to help develop an understandable story. 
%Bounegru \etal explore the potentials of narrative networks and summarize five ways extensively used in data journalism, %namely, \textit{Exploring Local Neighbourhoods}, \textit{Detecting Key Players}, \textit{Mapping Alliances and Oppositions}, \textit{Exploring the Evolution of Associations} and \textit{Revealing Hidden Ties}. 
%\name takes their research as the base of our topic generation and execlude the forth one, \textit{Exploring the Evolution of Associations} as \name does not support dynamic graph in current version.

\noindent
\textbf{G3. Design expressive and intuitive annotations.} 
Intuitive and expressive annotations are useful to emphasize important components on a graph, distinguish different types of facts, and provide explanations as well as context for the facts. Too much or too complex annotation designs would bring extra cognitive loads for general audiences. Therefore, it is important to design intuitive and expressive annotations to deliver the facts in an easy-to-understand manner.

%\name aims to deliver the facts to the audience with annotated graphs. 

%Rich information, on the other hand, may bring extra burdens for general audiences. 
%Therefore, intuitive and expressive annotations are required to meet such needs.
%TODO: which kind of annotations are intuitive &expressive (with explanation, visual metaphor/glyphs, etc.)
% To emphasize important components, concise and human-understandable annotations placed near the corresponding components are required due to the limited presentation space and the proximity principle\cite{hullman2013contextifier}. 
% When the annotations are connected to form a longer paragraph, the sentences need to be appropriately sequenced and connected by the proper conjunctions\cite{stolper2016emerging}.
% The annotations can provide necessary context information and guide users to the interesting features. For the first role, a longer paragraph is preferred to summarize the story and add necessary information\cite{stolper2016emerging}. 
% Annotations of varying lengths can play different roles and have different design requirements in narrative visualization. The long sentences can provide the necessary context information for the readers and are necessary to summarize the story generally.
% By contrast, the shorter labels can be closely related to the specific features and can guide the readers directly to them\cite{stolper2016emerging}. 
% Thus, the short annotations should 
% Thus the short annotations should meet the proximity to the focus components and be concise to reveal the crucial of the story due to the limited layout space and\cite{hullman2013contextifier}.
% Thus, the design goals of the long paragraph and short labels vary based on their functions. The long paragraph should be able to summarize the story generally and provide necessary context information. By contrast, 

%Ren \etal~\cite{ren2017chartaccent} expand the scope of annotation forms in visual storytelling from text to shape, highlights etc. To enhance expressiveness of the story, the system should support the diverse forms of annotations and combine them .
% Designing expressive/intuitive annotations to support the representation of different types of graph fact;
% Though slideshows are widely employed in data storytelling, especially in Calliope, annotated chart is a different genera, serving network narrative better. Firstly, network facts often have a proximity to the subject nodes and communities, when the annotations can be placed close to the corresponding network areas. Then, the annotated charts embed the network and provides a context for the audience. Furthermore, the static network does not have a temporal attribute, which is often used to order the data pieces in slideshows. Though there is no strict temporal order, a proper sequence in reading is helpful for the audience. Thus, the system should support a flexible reading sequence of the annotations in the network. 
% The system delivers the facts to the audience by the annotations, which is able to emphasize important elements in a graph, to distinguish different facts and to provide explanation as well as context for the facts. Ren \etal \cite{ren2017chartaccent} expand the scope of annotation forms in visual storytelling from text to shape, highlights etc.
% To enhance expressiveness of the story, the system should support the diverse forms of annotations and combine them .



\noindent
\textbf{G4. Present the annotated graph with good readability.}
Graph layout is crucial to improve readability. In addition to the aesthetic considerations in conventional graph layout (e.g., edge crossing), the visual information flow, the overlap and proximity of the annotations and the graph elements should be involved in the design process. Reducing overlapping could prevent the graph from being messy or causing ambiguity. The proximity principle indicates that annotations need to be placed visually near the related graph facts. When graph facts are added or deleted, the layout should be adjusted accordingly. Therefore, an effective layout algorithm is required to design an annotated graph with good readability.
%The overlap of the annotations and network elements should be alleviated, in that it can make the network messy and cause the ambiguity.
%Besides, proximity should be promoted in the layout process, meaning that the annotations need to be placed visually near the related network area. When a reader looks at an annotation, it is natural for him to examine the related nodes and communities. Thus, placing the annotations near the related elements can enhance the readability and provide a more entertaining reading experience to the audience. 
%verall, \name should ensure the readability of the annotated charts by a effective layout algorithm designed for both network and annotations. %The placement of annotations should also be considered in the layout process. 

\noindent
\textbf{G5. Enable flexible user interaction.} 
From our interviews and previous experience on human-machine collaborative systems, the fully automated approach can hardly meet all the requirements of users. The system should enable users to explore and modify the annotated graph content and style to satisfy user requirements for specific datasets and scenarios. Apart from manual adjustments, some recommendation functions such as potentially insightful facts, could also be provided to further facilitate the interaction process. 

% rich
% After presenting the automatic results to the audience, they sometimes still want to adjust or refine certain elements based on specific requirements. 
%Though, \name is designed to alleviate the barriers in network story creation, it is still necessary to involve human users in the generation process and allow users to edit the generated stories.
%In order to do so, \name should provide an interactive interface for user to view, edit and export the story. 
%The needs of real-time user interaction prioritize the efficiency issues in the system design. Thus, \name should implement efficient story generation and graph layout algorithms, by which the system can respond to the users after a reasonable time.


% \subsubsection{How to Extract Meaningful Facts From Network Data}
% When the automatic fact extraction from multi-dimensional data has been extensively studied in the recent years \cite{ding2019quickfacts, wang2019datashot}, the facts from graph data remain less explored. 
% The system generates the stories with meaningful and interesting facts embraced. A initial setup is to understand what facts can be measured as "interesting".
% Previous research on automatic fact extraction often apply a two-fold approach, which takes both the impact and significance into consideration, on the fact quality evaluation\cite{ding2019quickinsights, wang2019datashot}. In our scenario, the impact evaluates the importance of the fact subjects (community/node) against the whole graph when the significance measures the extend to which, the fact is surprising and interesting against a baseline in a stochastic fashion. Thus, the system should be able to mine the interesting facts from the graph in terms of significance and impact.



% \subsubsection{How to Present the facts by Annotations}
% Though slideshows are widely employed in data storytelling, especially in Calliope, annotated chart is a different genera, serving network narrative better. Firstly, network facts often have a proximity to the subject nodes and communities, when the annotations can be placed close to the corresponding network areas. Then, the annotated charts embed the network and provides a context for the audience. Furthermore, the static network does not have a temporal attribute, which is often used to order the data pieces in slideshows. Though there is no strict temporal order, a proper sequence in reading is helpful for the audience. Thus, the system should support a flexible reading sequence of the annotations in the network. 
% The system delivers the facts to the audience by the annotations, which is able to emphasize important elements in a graph, to distinguish different facts and to provide explanation as well as context for the facts. Ren \etal \cite{ren2017chartaccent} expand the scope of annotation forms in visual storytelling from text to shape, highlights etc.
% To enhance expressiveness of the story, the system should support the diverse forms of annotations and combine them .
% \subsubsection{How to Organize the Annotations}


% \subsubsection{How to Generate a Successive Story With Topicality and Cohesion}
% \subsubsection{How to Incorporate Users in the Design Process}
% The system supports the flexible editing of users and 

% \subsection{Design Goals}
% Graph Narratives

% Story Structure

% Tasks
% T1. Analyze graph dataset and discover interesting patterns

% T2. Apply a graph layout algorithm and manipulate the layout to make it conform to the communication context and to ensure it has the intended aesthetics and adequately communicates the intended message.	

% T3. Manipulate the visual attributes to make it conform to the communication context and to ensure it has the intended aesthetics and adequately communicates the intended message.

% T4. Add presentation aids that make the diagrams easier to read.

% T5. Introduce interesting communities in detail


% Design Requirements

% From the above discussion, we conclude the design goals summarized as follows.
% \begin{labeling}{alligator}
%     \item [\textbf{G1}] \textbf{Extract meaningful facts with significance and impact} The system should discover the meaningful patterns in the graph, which can be measured by impact and significance.

%     \item [\textbf{G2}] \textbf{Design expressive and intuitive annotations} 
%     Designing expressive/intuitive annotations to support the representation of different types of graph fact;
%     \item [\textbf{G3}] \textbf{Generate a successful story with topicality and cohesion} There are different factors contributing to the successful narration of a story. Here, we promote the importance of cohesion and topicality as the previous mentioned.

%     \item [\textbf{G4}] \textbf{Present the annotated graph with good readability}. The system should ensure the readability of the outputted poster by a effective graph layout algorithm for both graph annotations.
%     have an effective and efficient layout design for both graph and annotations, so the generated poster can be 
%     \item [\textbf{G5}] \textbf{Enable easy user interaction} The system should provide an interactive interface for user to view, edit and export the story. To fulfill it, the implementation of the system should take efficiencey issues into considerations, including both the efficiency of story generation and graph layout.

% \end{labeling}

% Generate 
% G1. Expressive/intuitive visualization design to support the representation of different types of graph fact
% Graph visualization, reducing edge crossings, remove overlap
% Reveal data fact with intuitive charts and meaningful narratives.

% G2. Easy to distinguish important graph elements (e.g., annotated nodes and communities) to facilitate the understanding of fact 
% Avoid conflict between the color indicating community and the highlighted color

% G3. Effective layout design for both graph visualization and annotations
% Reducing crossings of leaders with other leaders or graph links.
% Annotations have to be disjoint. And annotations cannot overlap with graph.
% Minimize the total length of all leaders (Place in the empty area near the node) and minimum the number of bends.
% Suitable order

% G4. Support the editing function. 
%Provide an overview of the entire network is an intuitive way to help users comprehend the data. 
%And recommend interesting subgraphs and enable users to have a deeper exploration. (Focus+Context: Fisheye)


-----------
The graph data fact bears a resemblance to the facts extracted from multi-dimensional data~\cite{wang2019datashot,shi2020calliope} in terms of the 5-tuple construction, while presents several major differences concerning the topology of the graph since the topology-based task is an essential task in graph analysis.
First, \name can select the subgraph based on topology information (e.g., one of the components divided by connected components).
Second, \name can explore the graph from different granularities (e.g., node-level, community-level).
Third, \name can extract topological features (e.g., node degree, community density) from different components of the graph.
For example, the graph data fact, {\it \{Extreme, \{\{country=China\}, \{country=Japan\}\}, \{none\}, \{degree\}, \{id=Wang\}\}}, describes that \emph{Wang} is an influential researcher based on the \emph{highest degree} between \emph{China} and \emph{Japan}. 
Similarly, the graph data fact, {\it \{Distribution, \{\{country=China\}\}, \{connected component\}, \{count\}, *\}}, divides the researchers in \emph{China} into various \emph{connected components} and studies the \emph{distribution} of different researcher groups' \emph{size (count)}.

% \subsection{Fact Formulation}
% Graph data include a set of nodes where edges connect some pairs of nodes. Commonly, nodes have several numerical or categorical attributes. Here, we take a bibliography network as an example, where nodes are the researchers with attributes (e.g., id, country, citations) and edges denote the co-authorship between researchers.

% Inspired by the concepts introduced in ~\cite{wang2019datashot,shi2020calliope}, a graph data fact represents a particular type of numerical measures in a specific subgraph. The nodes on the subgraph can be partitioned into communities.
% Formally, a graph data fact $f_i$ is denoted by a 5-tuple:
% \begin{equation*}
%     f_i = \{type, subgraph, partition, measure, focus\}
% \end{equation*}
% where \textbf{\textit{type}} describes the type of information referring to graph analysis tasks~\cite{lee_task_2006,pretorius2014tasks,ahn2013task} and facts taxonomy~\cite{yang_chen_toward_2009}. We collected 47 graph stories from data journalism and case studies of papers, summarized six common fact types (e.g., \textit{Extreme}, \textit{Outlier}, \textit{Rank}, \textit{Proportion}, \textit{Distribution}, \textit{Evenness}) to verify the validity of our method, more details are provided in the appendix. 
% \textbf{\textit{subgraph}} is defined as a set of data filters that zoom into a subgraph from the original graph in the following form: \begin{equation*}
%     \{\{\mathcal{F}[1]:\mathcal{V}[1]\},...\{\mathcal{F}[n]:\mathcal{V}[n]\}\}
% \end{equation*}
% where $\{\mathcal{F}[1]:\mathcal{V}[1]\}$ denotes a filter item with particular value $\mathcal{V}[i]$ on a specific field $\mathcal{F}[i]$. 
% The field $\mathcal{F}[i]$ can be the graph partition algorithm in addition to the categorical node attributes, and filed $\mathcal{F}[i]$ can take the same value as filed $\mathcal{F}[j]$ as long as $\mathcal{V}[i] \neq \mathcal{V}[j]$. Since even if the components are selected by different values, they are still connected by edges. 
% % TODO: ADD an example to explain filter f[i]: v[I], f[1]:v[1] -> f[I]: v[i]
% For example, {\it \{\{country=China\},\{country=Japan\}\}} is a subgraph that includes Chinese and Japanese researchers.
% \textbf{\textit{partition}} is used to divide the subgraph into a set of components (i.e., nodes or communities) based on the categorical node attributes or graph partition algorithm (e.g., connected component). To analyze the graph data from different granularity, \name explores the graph from the community level and node level. By default, the partition is none (i.e., node-level), where we treat each node as an independent component. 
% \textbf{\textit{measure}} is a numerical node attribute or a topological feature (e.g., node degree, community density). When the partitioned components are at the community-level, their value is derived as the summation of the node attribute.
% \textbf{\textit{focus}} highlights one (or some) of the partitioned components in the subgraph. For instance, for the \textit{Outlier} fact type, the focus component is the node with an outlier value. A detailed description of partition algorithms and topological features is provided in the appendix.

% The graph data fact bears a resemblance to the facts extracted from multi-dimensional data~\cite{wang2019datashot,shi2020calliope} in terms of the 5-tuple construction, but with several major differences. To be specific, we consider the topology of the graph since the topology-based task is an essential task in graph analysis.
% First, \name can select the subgraph based on topology information(e.g., one of the components divided by connected components).
% Second, \name can explore the graph from different granularity (e.g., node-level, community-level).
% Third, \name can extract topological features (e.g., node degree, community density) from different components of the graph.

% To facilitate understanding, we provide two specific examples. The graph data fact, {\it \{Extreme, \{\{country=China\}, \{country=Japan\}\}, \{none\}, \{degree\}, \{id=Wang\}\}}, describes that \emph{Wang} is an influential researcher based on the \emph{highest degree} between \emph{China} and \emph{Japan}. 
% % {\it \{\texttt{Extreme}, \{\{\texttt{Country=China}\}\}, \{\texttt{None}\}, \{\texttt{citations}\}, \{\texttt{id=Wang}\}\}}
% Similarity, the graph data fact, {\it \{Distribution, \{\{country=China\}\}, \{connected component\}, \{count\}, *\}}, divides the researchers in \emph{China} into various \emph{connected components} and studies the \emph{distribution} of different researcher groups' \emph{size (count)}.
% %{\it \{\texttt{Distribution}, \{\{\texttt{Country=China}\}\}, \{\texttt{Connected component}\}, \{\texttt{COUNT}\}, \texttt{*}\}}

% subspace
% \paragraph{Subgraph selection.} Given an audience-provided graph $G=\{V,E\}$ where $V$ and $E$ are the set of nodes and edges respectively, \name zooms in on a subgraph $G^{\prime}=\{V^{\prime},E^{\prime}\}$ from the original graph $G$ (i.e., $G^{\prime}\subseteq G$) via a selection strategy $\phi$ (i.e., $G^{\prime}=\phi(G)$) which can be instantiated as two variants: topological detection and node attribute filtering. Topological detection exploits the critical components of the $G$ to compose the target subgraph $G^{\prime}$. \name adopts, for example, k-core~\cite{seidman1983network} to extract the cohesive subgraph $G^{\prime}$. 
% For the node attribute filtering, \name queries the node set $V^{\prime}$ whose attributes satisfy $\texttt{attribute}_i=\texttt{value}_i$ (e.g., $\texttt{domain}=\texttt{visualization}$.). Then \name selects edges $E^{\prime}\subseteq E$ whose source and target nodes both belong to the $V^{\prime}$.
% partition
% \paragraph{Graph partition.} Towards the selected graph $G^{\prime}$ from the last step, \name partitions it into a set of components $\{G^{\prime}_i\}$ for further comparison based on the a graph partition function $\psi$ (i.e., $\{G^{\prime}_i\}=\psi(G^{\prime})$), where $G^{\prime}_i$ denotes the $i$-th component from the selected graph $G^{\prime}$. Here, to provide analysis of the graph data from different resolutions, \name explores the selected graph $G^{\prime}$ from community level (i.e., $\{G^{\prime}_i\}$ is the set of subgraphs) and node level(i.e., $\{G^{\prime}_i\} = V^{\prime}$) by multiple choices of $\psi$. The node-level partition is straightforward that every component $G^{\prime}_i$ is consisted by a single node. For the community-level graph partition, a line of the candidate strategies is similar as the aforementioned node attribute filtering with different candidate attribute values $\{\texttt{value}_i\}$ w.r.t. a specific attribute. For instance, on a social network, the attribute \texttt{Gender} has candidate values \texttt{Male}, \texttt{Female}, and \texttt{Others} which can be used to partition the selected graph $G^{\prime}$. The other line of community-level graph partition strategies is to utilize the graph topology to split the given $G^{\prime}$ into multiple cohesive subgraphs. For instance, \name can split the given $G^{\prime}$ into multiple connected components (if applicable). Detailed description of topological split strategies are provided in Appendix~\ref{appendix:partition}.
% measure
% \paragraph{Feature calculation.} In this step, with the partitioned graphs $\{G^{\prime}_i\}$, \name selects a feature $\rho$ to extract corresponding feature values from every partitioned graph: $\{G^{\prime}_i\}\rightarrow \{\rho(G^{\prime}_i)\}$. Specifically, the selections of $\rho$ fall into four scenarios which are the combinations of node-level/community-level partition v.s. attribute value/topological feature. When the partitioned graphs are node-level (i.e., $\{G^{\prime}_i\} = V^{\prime}$), $\rho$ can be either the node attribute (e.g., \# of citations) or the node topological feature (e.g., node degree, pagerank score~\cite{page1999pagerank}). When the partitioned graphs are community-level (i.e., $\{G^{\prime}_i\}$ is the set of subgraphs), the $\rho$ can be either the summation of the node attribute from every subgraphs (e.g., the summation of annual income) or the community topological feature (e.g., density of every subgraph). The detailed selections of $\rho$ are provided in Appendix~\ref{appendix:feature}.



% \subsection{Fact Scoring} 
% To extract meaningful facts (\textbf{G1}), we evaluate the importance of a graph data fact $f_i$ from two perspectives,  \textbf{\textit{impact}} and \textbf{\textit{interestingness}}, based on the preview research~\cite{ding2019quickinsights,tang2017extracting} on auto-insight. When more nodes and edges are involved, a greater impact is considered for this fact. $G(V,E)$ denotes the input graph $G$ where $V$ is a set of nodes and $E$ is a set of edges, and $G_{i}(V_{i},E_{i})$ represents the selected subgraph of $f_i$ where $V_{i} \subseteq V$ and $E_{i} \subseteq E$
% . 
% Thus, \name obtains \textbf{\textit{impact}} as follows:
% \begin{equation}
%     impact(f_i)=\max(\frac{|V_{i}|}{|V|},\frac{|E_{i}|}{|E|})
% \end{equation}
% where $|\cdot|$ denotes the number of elements of the given set. 
% For the \textbf{\textit{interestingness}}, \name evaluates it based on the statistical properties with a fact type-specific function. We follow the idea of existing auto-insight work~\cite{ding2019quickinsights,tang2017extracting,wang2019datashot,shi2020calliope} to design the function $interestingness(f_i)$.
% % For example, for the insight type \emph{evenness}, the null hypothesis is defined that the extracted value from different partitioned graphs should be equal. 
% The detailed descriptions of $interestingness(f_i)$ score for different fact types are provided in the appendix. 
% As only the facts that are both impactful and interesting would be considered meaningful, the final \textbf{\textit{score}} of graph data fact is computed as: 
% \begin{equation}
%     score(f_i) = impact(f_i)\times interestingness(f_i)
% \label{eq:score}
% \end{equation}

% In general, the search space is defined by four aforementioned functions $\{\phi,\psi,\rho,\texttt{type}\}$ and every insight extracted can be unambiguously represented by a specific set of $\{\phi,\psi,\rho,\texttt{type}\}$. Together with the corresponding \texttt{focus} and \texttt{score} values, the hextuple $\{\phi,\psi,\rho, \texttt{type}, \texttt{focus}, \texttt{score}\}$ contains all the information needed for downstream tasks.

% For the importance of mined patterns, \name evaluates it from two perspectives, \texttt{impact} and \texttt{interestingness}. Here we assume that the more nodes and edges are involved into the detected pattern, the greater impact this pattern holds. Thus, \name obtains \texttt{impact} as follows:
% \begin{equation}
%     \texttt{impact}=\max(\frac{|V^{\prime}|}{|V|},\frac{|E^{\prime}|}{|E|})
% \end{equation}
% \noindent where $|\cdot|$ denotes the size of given set. For the \texttt{interestingness}, \name evaluates it based on the extracted features $\{\rho(G^{\prime}_i)\}$ with a fact type-specific function $\kappa_{\texttt{type}}$: $\texttt{interestingness}= \kappa_{\texttt{type}}(\{\rho(G^{\prime}_i)\})$. We follow the idea of existing auto-insight works~\cite{ding2019quickinsights,tang2017extracting} to design the function $\kappa_{\texttt{type}}$ as $1-p$ where the $p$-value is calculated against an insight type-specific null hypothesis. For example, for the insight type \emph{Categorization}, the null hypothesis is defined that the extracted feature $\{\rho(G^{\prime}_i)\}$ from different partitioned graphs should be equal. In addition, to assist visualization, for a part of insight types, \name highlights one (or some) of the partitioned components and name it (or them) as \texttt{focus}. For instance, for the insight type \emph{Proportion}, the subgraph whose feature dominates all the extracted features $\{\rho(G^{\prime}_i)\}$ is set as the \texttt{focus}. Detailed description of $\kappa_{\texttt{type}}$ and \texttt{focus} for different insight types are provided in Appendix~\ref{appendix:interestingness}. The final score of extracted insight can be computed as: $\texttt{score} = \texttt{impact}\times\texttt{interestingness}$.

% In general, the search space is defined by four aforementioned functions $\{\phi,\psi,\rho,\texttt{type}\}$ and every insight extracted can be unambiguously represented by a specific set of $\{\phi,\psi,\rho,\texttt{type}\}$. Together with the corresponding \texttt{focus} and \texttt{score} values, the hextuple $\{\phi,\psi,\rho, \texttt{type}, \texttt{focus}, \texttt{score}\}$ contains all the information needed for downstream tasks.

% {\em Remarks.} The generated hextuple $\{\phi,\psi,\rho, \texttt{type}, \texttt{focus}, \texttt{score}\}$ bears high-level resemblance with the insights extracted from multi-dimensional data~\cite{ding2019quickinsights,tang2017extracting} but with several important differences. First, \name can select the mining scope and split the selected subgraph based on topology information (i.e., topological detection strategy for subgraph selection and topological split of the selected graph $G^{\prime}$); second, \name can explore the given mining scope from different resolutions (i.e., node-level and community-level partition); third, \name can extract topological features (e.g., node degree, graph density) from different components of the graph. In the end of this subsection, we provide several examples of extracted insight and represent them as $\{\phi,\psi,\rho,\kappa\}$ (the \texttt{focus} and \texttt{score} can be computed based on the first four elements). We assume that the input network is a bibliography network whose nodes are the researchers with node attributes such as country, institution, \# of citations. The edges denote co-authorship between researchers. 

% \noindent \textbf{Example 1:} $\{k\textrm{-core=}5, \textrm{Country}, \textrm{Density}, \textrm{Categorization}\}$. \name focuses on a subgraph $G^{\prime}$ whose node degree is at least $5$. Then, our system evaluates that whether the collaboration \emph{density} of researchers from different \emph{countries} are distributed consistently.

% \noindent \textbf{Example 2:} $\{\textrm{Country=the US}, \textrm{Node}, \textrm{\# of citations}, \textrm{Distribution}\}$. \name explores that whether the \emph{number of citations} of researchers from \emph{the US} follows the power-law distribution.

% \noindent \textbf{Example 3:} $\{\textrm{Country=the US}, \textrm{Connected component}, \textrm{Count}, \textrm{Proportion}\}$. \name divides the US researchers into various \emph{connected components} and studies that whether there exists a dominant group of researchers whose \emph{size} (i.e., Count) is larger than $50\%$ of the total number of researchers. 

To extract meaningful and interesting facts (\textbf{G1}), we evaluate the importance of a graph data fact $f_i$ from two perspectives, \textbf{\textit{impact}} and \textbf{\textit{interestingness}}, based on the previous research~\cite{ding2019quickinsights,tang2017extracting} on auto-insight. If more nodes and edges are involved, a greater impact is considered for this fact. $G(V,E)$ denotes the input graph $G$ where $V$ is a set of nodes and $E$ is a set of edges. $G_{i}(V_{i},E_{i})$ represents the selected subgraph of $f_i$ where $V_{i} \subseteq V$ and $E_{i} \subseteq E$. 
Thus, \name obtains \textbf{\textit{impact}} as follows:
\begin{equation}
    impact(f_i)=\max(\frac{|V_{i}|}{|V|},\frac{|E_{i}|}{|E|})
\end{equation}
where $|\cdot|$ denotes the number of elements of the given set. 
For the \textbf{\textit{interestingness}}, \name evaluates it based on the statistical properties with a fact-type-specific function. We follow the idea of existing auto-insight work~\cite{ding2019quickinsights,tang2017extracting,wang2019datashot,shi2020calliope} to design the function $interestingness(f_i)$.
The detailed descriptions of $interestingness(f_i)$ score for different fact types are provided in Table \ref{tab:fact-overview}. 
Since the facts that are both impactful and interesting would be considered meaningful, the final \textbf{\textit{score}} of graph data fact is computed as: 
\begin{equation}
    score(f_i) = impact(f_i)\times interestingness(f_i)
\label{eq:score}
\end{equation}
------------------

% To create a graph story poster, three steps are required with our prototyping system. For the first step, the user can click to upload a json file or drag the json file to the uploading area. Then the editing page (Fig.~\ref{fig:interface}) appears to allow further adjustment of the generated poster. The title and the text summary of the graph story are shown at the top of the poster with the legend. The generated graph with annotations is shown at the center of the poster, in which a user can remove an annotation or change the generated narrative order number based on his/her own preferences. Each fact is captioned by a generated text description and some of them are visualized with a chart, for instance, bar chart for the rank and pie chart for the proportion. When a node/community has more than one fact, the facts can be shown in one annotation. Each annotation is connected with its subject by a line, and they also share the same color. The graph summary includes distribution and evenness, which is shown at the bottom of the poster. Each summary is visualized by a histogram and captioned by a generated text description. The textual representations of the poster are also editable.
% overview也有stroy editor

We introduce the system interface and how to edit and refine the generated annotated chart (\textbf{G5}). To begin with, the user can upload the JSON format graph data and click the generation button. 
Then the main interface (Fig.~\ref{fig:interface}) consisting of the annotated graph and the configuration panel, is shown. 
\rv{TODO} % TODO: 版式在case study补充
In the annotated graph (Fig.~\ref{fig:interface}-1), the title and the text summary (Fig.~\ref{fig:interface}-1(a)) are shown at the top with the annotation legend (Fig.~\ref{fig:interface}-1(b)). 
The graph (Fig.~\ref{fig:interface}-1(c)) with annotations is shown at the center.
The graph summary (Fig.~\ref{fig:interface}-1(d)), including distribution and evenness, is shown at the bottom. 
Users can interactively remove, edit and add a fact either by the fact editor (Fig.~\ref{fig:interface}-2). By double-clicking on a particular node or community, users can check the recommended data facts focused on the node or community (Fig.~\ref{fig:interface}-3). The narrative order and text descriptions of the annotations can also be modified. In addition, users can manually adjust the locations of nodes, communities, and annotations.
To find a specific node, users can search the node name in the search box on the configuration panel (Fig.~\ref{fig:interface}-4).
In the fact organization zone (Fig.~\ref{fig:interface}-5), the user can set the topics and the partition algorithm, and regenerate the annotated graph.
Users can also change ``Style'' and ``Layout'' (Fig.~\ref{fig:interface}-6,7) to adjust presentation style and layout.
To further customize the annotated graph, users can modify the style of node and link (Fig.~\ref{fig:interface}-8).
After all the adjustments are made, users can export the generated visualization by clicking the ``Export'' button (Fig.~\ref{fig:interface}-9).


-----------



\textbf{\textit{Network Integrity}} measures the network coverage of the selected facts given by:
\begin{equation}
I(S) = \frac{|\bigcup V_N|}{|V|}
\end{equation}
where $V_N$ refers to the focus nodes of all the facts in the narrative $N$. A story with a higher integrity score can cover more nodes and represent more general network patterns.

After specifying the rewards evaluating the selected facts, we propose two cost functions to evaluate the relations of the facts.
\textbf{\textit{Cost Functions}} correspond to the two relation types we set previously. 
The cost for logical relations is calculated based on the transition probability proposed by Shi \etal~\cite{shi2020calliope} as follows:
\begin{equation}
NC(r) =  \frac{1}{ 1 + p(r)}
\end{equation}
where $p(r)$ is the probability that the relation $r$ has. 
We represent the cost by the inverse of the likelihoods' harmonic average in order to normalize the probability distribution and prevent the result dominated by some overlarge items.

Then, the topological cost of a relation is given by:
\begin{equation}
TC(r) = \begin{cases}
      0 & \text{if } r.f_n.focus \text{ is same with } r.f_p.focus\\
      1 & \text{if } r.f_n.focus \text{ is connected with }  r.f_p.focus\\
      \infty & \text{if }  r.f_n.focus \text{ is not connected with } r.f_p.focus\\
    \end{cases}       
\end{equation}
where $r$ is the relation. Facts related topologically (e.g., within the same node, with a connected edge) can relieve readers' burdens and promote readability. 
After obtaining the two costs separately, we formulate the overall cost by:
\begin{equation}
C(r) = \frac{\gamma_1 + \gamma_2}{\frac{\gamma_1}{TC(r)} + \frac{\gamma_2}{NC(r)}}
\end{equation}
We represent the cost by the harmonic mean of the two costs weights $\gamma_1, \gamma_2$ to prevent cost calculation being dominated by the bigger cost. Besides, the harmonic mean can also resolve the issues of the infinite topological cost caused by the facts without any topological connection. 


\subsection{Text Generation} \label{sec:textgeneration}
\name includes a text summary of the graph story and a series of annotations for the accompanying facts. To generate comprehensible text annotations (\textbf{G2}), we involved the graph mining experts in our development phase and employ a template-based text generation method. 
The experts created a set of annotation examples for the different types of facts. After transforming those annotations into the templates, we also invited the experts to read the generated text and further fine-tune them. We design various templates for different types of facts, with the empty slots filled by partition methods, measures and focus subjects. 

To improve the readability of the text annotations, we introduce measure translation and conjunctions (e.g., similarity, to elaborate) in the templates. The graph data facts comprises a series of topological measures such as density, triangle participation rate (TPR). Those will cause extra burdens for the readers without network background. Thus, we describe them in a more understandable way, while preserving the original terms in the annotations. For example, density, inside edge number and TPR all reflect the internal cohesion of a community in the network. 
The templates include a slot called \{Measure Translation\} which can be filled by the converted measure description as the appendix shows. 
For instance, if a community reaches the extreme of TPR, \name will describe it as \textit{The community is a cohesive community based on the highest triangle participation rate.}
Experts agree that though the measure translation is not rigorously stated, the enhanced comprehensibility outweighs the drawbacks.
In the text summary, using conjunctions can imply the relationship between two successive sentences and improve the fluency of the text. We generate the conjunctions based on the narrative relations such as the \textit{Similarity} of the facts. The detailed templates can be found in the appendix.
-----------------------
\subsection{Fact Annotation Encoding} \label{sec:visual}

Referring to the design space from \cite{ren2017chartaccent}, \textit{annotation target} and \textit{annotation form} need to be considered when designing annotations.   
\textit{Annotation target} is a data item/set (in our case, node/community), which is the focus of the data facts.
Regarding the design of \textit{annotation form}, we take a combination of various annotation forms (i.e., text, highlights, glyphs as shapes, and visualizations as images) to emphasize the essential elements, distinguish different fact types and provide expressive explanations (\textbf{G3}).

As mentioned in Section \ref{sec:factdiscovey}, we summarized six fact types, four of which are with focus (e.g., \textit{Extreme}, \textit{Outlier}, \textit{Rank}, \textit{Proportion}) and two without focus (e.g., \textit{Distribution}, \textit{Evenness}). For a fact with focus, we highlight its focus (e.g., node, community) on the graph and connect the focus to the annotation with leader lines. It is worth noting that when the focus is a node, we replace the node with a well-designed glyph to denote its fact type. \textit{Rank} and \textit{Proportion} facts are denoted by annotations with both visualizations and generated text descriptions, while \textit{Extreme} and \textit{Outlier} facts are presented with text-only annotations. For a fact without focus, we consider it as graph-level information and therefore present it as a captioned chart in the \textit{graph summary} below the poster. 
% from short paper
Apart from different presentation forms, other considerations have been taken into account when designing the annotations, such as the style of the leader lines, various highlighting methods for facts from different granularities. For example, for the community-level annotations, three design alternatives were considered (Fig.~\ref{fig:design}). 
We discuss with the same four journalists from previous expert interviews to evaluate the aesthetics and expressiveness of various design choices. 
Considering the clarity of annotations on different backgrounds, the separability from the node-level annotations, and the mapping with the leader lines, Fig.~\ref{fig:design}(c) is finally selected. 
In addition, we align facts with the same focus as a single annotation for aesthetics and simplicity. To restrict the annotations’ area, the annotation is limited to a maximum width and height. When the text exceeds the limited width and height, it is resolved by decreasing the font size. %Also, we will avoid leaving large gaps caused by text line breaks.



%%%%%%%%%%%%%%%%%%% intro
%However, it is not an easy task to discover interesting insights from graph visualization. First, it requires users to be equipped with adequate data analysis skills and domain knowledge. Second, even experienced analysts need to spend much time and effort assessing the interestingness and significance of a huge number of potential graph insights. Therefore, a means to automatically discover graph insights is required by both general users and domain experts.

%\rv{contribution and focus on explanatory rather than narrative story}

Graph data are applied in a wide range of domains, from social network analysis~\cite{freeman2004development} to the study of disease transmission pathways~\cite{campbell2017detailed}. Over the past few decades, graph visualization and visual analysis have been extensively studied~\cite{herman2000graph,lee_task_2006}. The growth of social networks and social media in recent years has drawn even more interest to the exploration of insightful patterns in graph data~\cite{nettleton2013data}. Such insights from network diagrams could assist in understanding the relationship among different entities and groups. Moreover, it is important for data journalists to effectively deliver and present such insights in an intuitive and expressive format. %However, creating such graph visualizations is not an easy task for data journalists or designers. %They need to first derive the insight from the original dataset, then use a graph visualization software to draw an initial visualization, choose the important nodes/groups, add annotations, fill in the annotation content and adjust the layout, revise the overall visual representation, and finally get the output. This process usually involves multiple co-workers from different background, or an experienced data journalist who is equipped with all those techniques and knowledge.

Nevertheless, existing tools built for graph visualizations may not sufficiently support the whole insight discovery, organization and presentation process. First, it is not easy task for data journalists or domain experts to derive valuable insights. Current work requires users to be equipped with adequate data analysis skills and domain knowledge. Even experienced analysts need to spend much time and effort assessing the interestingness and significance of a huge number of potential graph insights. To explore graph insights, data journalists and domain experts usually need to utilize standard graph visualization software or develop specific systems and manually select insightful facts. Given the amount of potentially interesting graph insights and the manual cost for such exploratory visual analysis, it is time-consuming to conduct this tedious task, especially when the end users have limited time and inadequate expertise or domain knowledge~\cite{ding2019quickinsights}. Second, after exploring graph insights, it not also non-trivial to effectively present such derived data facts in graph visualization, in order to deliver core messages around a meaningful topic to the end users~\cite{lee2015more,srinivasan_augmenting_2019}.
Despite the extensive studies on graph visualization~\cite{nobre2019state}, there is limited support to help create visual narratives of graph data facts. Annotated visualization is a suitable narrative form since graph data facts are highly related to the graph structure, which requires to present the location information and semantic meaning at the same time.
It can be a laborious task when the data becomes large and complex, considering the huge design space for organizing visual elements and effective graph layout. Therefore, an automatic annotation framework for the discovery and presentation of graph insights should be provided.
%journalists need visual interfaces that cater to the exploratory nature of their investigative activities. 

%Creating such graph visualizations with annotations is not an easy task for data journalists or designers, especially those without much technical background. They need to first derive the insight from the original dataset, then use a graph visualization software to draw an initial visualization, choose the important nodes/groups, add annotations, fill in the annotation content and adjust the layout, revise the overall visual representation, and finally get the output. This process usually involves multiple co-workers from different background, or an experienced data journalist who is equipped with all those techniques and knowledge

%1-insight extraction challenge
%However, it is challenging to discover reliable and interesting insights from graph data. First, it requires users to be equipped with adequate data analysis skills and domain knowledge. Second, even experienced analysts need to spend much time and effort assessing the interestingness and significance of a huge number of potential graph insights. To explore graph insights, data journalists and domain experts usually need to utilize standard graph visualization software or develop specific systems and manually select insightful facts. Given the amount of potentially interesting graph insights and the manual cost for such exploratory visual analysis, it is time-consuming to conduct this tedious task, especially when the end users have limited time and inadequate expertise or domain knowledge~\cite{ding2019quickinsights}.

%2-organization and presentation challenge
%Apart from the automatic discovery of graph insights, another urgent need is to effectively present such derived data facts in graph visualization, for the purpose of deriving a readable data story to the end users~\cite{lee2015more,srinivasan_augmenting_2019}. Despite the extensive studies on graph visualization~\cite{nobre2019state}, there is limited support for visual storytelling of graph data facts. Annotated visualization is a suitable narrative form since graph data facts are highly related to the graph structure, which requires to present the location information and semantic meaning at the same time. It can be a laborious task when the data becomes large and complex, considering the huge design space for organizing visual elements and effective graph layout. Therefore, an automatic annotation framework for the discovery and presentation of graph insights should be provided.

%However, three key challenges must be addressed to discover such graph insights and present them effectively in an annotated graph visualization. The first challenge is to extract reliable and interesting insights from graph data. Some existing work has studied the automatic generation of insights from multi-dimensional data. Such generated insights, however, have no logical ties, which makes it difficult for users to assemble a coherent story together; the second challenge, therefore, is to organize extracted facts into meaningful graph topics. The final challenge lies in the expressive visual presentation of graph insight story on an annotated chart. Various visual elements such as marks, annotations, and graph visualization complicate the layout consideration. %%In addition, a more flexible layout algorithm should be proposed to allow dynamic editing of existing graph facts and annotations.

To tackle these two challenges, we present \name, a novel framework to create annotated narrative visualizations with insights automatically discovered from graph data. The framework consists of a fact discovery module, a fact organization module, and a visualization module. The fact discovery module automatically extracts interesting patterns and formulates them into facts. The fact organization module gradually selects facts and organizes them around a meaningful topic, which is guaranteed by the topic-evidence-explanation structure. The visualization module presents the selected facts as a series of expressive annotations on the graph. An annotation-aware graph layout algorithm is designed to place the graph visualization and annotations properly.

With the proposed framework, we are able to significantly reduce the efforts involved in discovering graph insights, effectively creating expressive presentations. We then developed a prototype system with interactive features such as editing to accommodate different user purposes. Finally, we conducted case studies to demonstrate the usability of our system and an in-lab user study to verify the generated annotated graphs by \name from various perspectives. 

%With the proposed framework, we are able to significantly reduce the efforts involved in discovering graph insights, creating expressive presentations, and to make them accessible to users without much expertise or domain knowledge. We then developed a prototype system with interactive features such as editing to accommodate different user purposes. Finally, we conducted case studies to demonstrate the usability of our system and an in-lab user study to verify the generated annotated graphs by \name from various perspectives. 


The contributions of this paper are as follows:
\begin{itemize}
\itemsep -1mm
    \item We present a framework to create annotated visualizations with insights automatically discovered and organized from graph data.
    \item We design a three-step layout algorithm for graph visualization and annotation placement to deliver meaningful graph narratives.
    \item We develop an interactive prototype system and apply real-world data to demonstrate its usefulness. Two case studies and a user study are conducted to reveal its potential benefits.
\end{itemize}

%Fig1. story expansion -> narrative expansion

%It would be desirable if, over the process of exploration and analysis, the visualization system suggests important areas and features to select and label, for the purpose of deriving a data story to use in subsequent tasks or presentations.

%To begin with, we derive several design goals for building an automatic annotation framework from the survey of graph visualization~\cite{purchase2000effective, bennett2007aesthetics} and the interviews with domain experts. Then, we use a similar fact definition for graph data, inspired by QuickInsight~\cite{ding2019quickinsights}, and further extend the scoring measures to the story-level. Next, we arrange the scored insights according to a topic-evidence-explanation structure, in which evidence insights are selected by topic-aware algorithms and explanation insights are selected by a greedy search strategy. To improve the time efficiency, we further apply a bandit strategy, which explores different topics within a time budget before exploiting the most promising topic.
%Finally, we consider seven constraints to automatically optimize the layout so that the graph facts can be presented in a way that is easy to read. 

%Finally, it is important to automatically customize the graph visualization layout so that the results can be presented in a way that is easy to read. We consider seven constraints in the layout process, which are carried out in three steps: (1) creating the initial graph layout to match appropriate reading flows, (2) searching for blank areas and placing corresponding the annotation, (3) optimizing the final layout to avoid overlapping and crossing.
%Meanwhile, interactive features such as editing are provided to accommodate different user purposes.



    
%%%%%%%%%%%%%%%%%%%
%\section{User Study}
% The overall goal of our evaluation was to evaluate
% 1)fact generation: whether Calliope-Net can help users find insightful facts
% 2)story generation: whether the story sequence generated can help users understand the facts
% 3)annotation layout: whether the final presentation is effective/aesthetic/expressive, compared with manual layout




%(1) the data fact (\textit{Insightful, Comprehensive}), (2) the placement of the annotations (\textit{Reasonable}) and the annotated graph's layout (\textit{Aesthetics}), (3) the overall experience (\textit{Comprehension, Engagement, Memorability}).

\subsection{Feedback}
Participants generally assessed annotated graphs with positive feedback, as shown in Fig.\ref{fig:evaluation}. Compared annotated graph generated with created by domain experts, there is no significant difference ($p>.05$). 
Generally, all the participants agreed that the annotated graphs automatically generated are as good as or even slightly better than those given by experts in terms of reasonable annotation layout. However, in terms of Logicality and Memorability, domain experts received more positive feedback than \name. % Comprehension
We analyze subjective feedback from participants to have a better understanding of the reasons for their ratings.

\textbf{Sufficient and Insightful Data Facts.} All the participants agreed that the extracted data facts were meaningful. P7 commented that \textit{``I was excited to find out about the relationship of the main characters in the TV series, even though I had not watched it before.''}. Moreover, the participants reported that 
\textit{``the information is rich as the graph covers many analysis perspectives''}(P4). E5 mentioned that \textit{``[The annotated graph] offers extensive information from a data perspective which can help quickly understand the data''}. E3 observed that \textit{``the annotated graph contains multiple levels of detail, covering the overall graph-level information as well as the community-level and the node-level insights''}. P8 also felt that \textit{``the number of annotations and the amount of information shown on the graph is adequate''}. 

%\textbf{Comprehensible and Rational Graph Story.}
%All the participants agreed that the generated story’s logic was clear and easy to understand, \textit{``the story is coherent''}(E8).
%P2 commented that \textit{``the description is fluent. I have no trouble reading them in the given order''}.
%E1 said that \textit{``the story starts with the essential node and follows the community that contains it, ..., the narrative, from the details to the overview, is logical''}.
%Most participants noted that \textit{``the graph is well illustrated with detailed annotations''}(P1-P2, P5-P8, E1-E6, E9), \textit{``with the help of annotations, information about the node's degree, community's density are more explicit''}(E2). They also mentioned that clear logic improved story comprehension (P8, E3, E7). Compared the annotated graph generated by \name with that created by domain experts, we found experts were accustomed to creating narratives from overview to detail, while our algorithm focused more on the relationship between facts. It is interesting to note that for the same story, E1 felt that the structure ``detail-overview-detail'' makes sense, while P4 said \textit{``it would be better if the rank fact involving the three communities was at the beginning''}.

\textbf{Expressive Visualizations and Effective Layout.} 
The participants appreciated the layout of the annotations, \textit{``the annotations make use of the blank space and do not overlap the important details in the graph''}(E2). P5 commented that \textit{``the distance from the annotation to the node is appropriate. I can easily locate the annotations with the corresponding graph elements''}. E5 noted that \textit{``the annotations are placed from top to bottom. This placement is reasonable and fits normal reading habits''}. While most participants agreed the generated layout was elegant, we found that the annotated graphs created by experts would perform better in terms of the overall graph balance.

\textbf{Satisfactory Overall Experience.}
All the participants agreed that the annotated graph was clear and easy to understand. Compared the annotated graph generated by \name with that created by domain experts, we found experts were accustomed to creating narratives from overview to detail, while our algorithm focused more on the relationship between facts. Most participants noted that \textit{``the graph is well illustrated with detailed annotations''}(P1-P2, P5-P8, E1-E6, E9), \textit{``with the help of annotations, information about the node's degree, community's density are more explicit''}(E2). They also mentioned that the selection of related data facts and the organization improved the general comprehension and memorability(P8, E3, E7). 





%%%%%case study%%%%%%
To validate the framework and demonstrate the usefulness of \name, we performed case studies with two real-world datasets. %The first was conducted with two graph experts from a famous university. The second was done with an experienced visualization researcher. In both studies, the experts were asked to read the generated story and interact with our system. From their feedback and our observations, \name shows its usefulness and expressiveness.

\subsection{Case Study One: Les Misérables}
The \textbf{\textit{Les Misérables Co-occurrence}} network dataset\cite{knuth1993stanford} has 77 nodes and 254 edges. Each node represents a character, and an edge connects two characters whenever they appear in the same chapter of Hugo's novel Les Misérables\cite{enwiki:1006098025}. 
With \name, the experts generated annotated graphs on two different topics,  \textbf{\textit{Exploring Local Neighbors}} and \textbf{\textit{Revealing Hidden Ties}}, respectively.
Fig.\ref{fig:casestudy}(a) shows a generated graph which topic is \textbf{\textit{Revealing Hidden Ties}}. The annotated graph illustrates that the protagonist, Valjean, is the bridge connecting two communities (in pink and purple) partitioned by Clauset-Newman-Moore greedy modularity maximization~\cite{clauset2004finding}, as he is the node with the highest degree between both communities (\textit{Annotation 1}). 

According to the PageRank score, Valjean is an influencer in the novel (\textit{Annotation 1}). The community containing Valjean is also quite influential, as it is the largest community with $33.77\%$ of the number nodes of the entire network (\textit{Annotation 2}). However, the node Labarre is an outlier in terms of both degree and PageRank score (\textit{Annotation 3}). Meanwhile, the purple community is a cohesive community based on the inside edge number accounted for $35.48\%$ (\textit{Annotation 4}).
The node Gavroche within the purple community is also an influencer, shown by the fact that he has the highest eigenvector centrality (\textit{Annotation 5}). Finally, the \textit{Graph Summary} at the bottom shows the distribution of node's degree, eigenvector centrality, and PageRank score between the pink and the purple communities. For example, the histogram showing the distribution of the eigenvector centrality illustrates that a portion of the nodes in both the pink and purple communities are essential to the connectivity of the two communities.

Based on discussions with the experts during the generation, reading, and system interaction sessions, we received much valuable feedback. Both experts agreed the generated graphs contained interesting data insights, and the information annotated is convincing. One expert mentioned that \textit{``it's great that the selected topic and annotations contain information about the communities. In network analysis, there are quite a few community-related tasks."}.  The other commented that \textit{``the graph summary is useful to know that the graph is unevenly distributed and there are a few nodes which are particularly important.''} They also mentioned that \textit{``I appreciate grouping multiple insights that relate with one single node into one annotation, which is elegant and easy to understand.''}

Regarding the system, experts mentioned that automatic annotations helped gain an initial sense of the network, \textit{``it's much smarter than I have imagined"}. They praised the easy-to-use generation and editing features. Experts were delighted to see that communities can be highlighted when hovering on and that communities can be moved and remapped. One expert dragged all the small communities to the corners and explained, \textit{``I would prefer to put aside uninterested communities and focus more on those that have certain graph structures.''}

\subsection{Case Study Two: Stack Overflow}
The \textbf{\textit{Stack Overflow Tag}} network dataset \cite{stackoverflow} includes 115 nodes and 245 edges, where each node is a technology tag and an edge represents two tags appearing together on developers' \textit{Developer Stories}. With this dataset, the experts explored two annotated graphs generated by our prototype system. Fig.\ref{fig:casestudy}(b) shows one graph narrative about \textbf{\textit{Detecting Key Players}}, aiming at discovering influential technologies in the tech ecosystem. The graph shows that JavaScript is an influential node according to frequency (\textit{Annotation 1}); jQuery is the node with the highest degree and eigenvector centrality (\textit{Annotation 2}); Linux is also the node with highest PageRank score (\textit{Annotation 3}). Similarly, the top three influencers ranked by PageRank score are Linux, C-Sharp, and jQuery (\textit{Annotation 4}). Furthermore, the C-Sharp node has the highest degree in its community (calculated via a cluster walktrap) (\textit{Annotation 5}). The \textit{Graph Summary} shows the distribution of technology's frequency, degree, eigenvector centrality, and PageRank score.

The expert provided abundant feedback in the whole process. He enjoyed reading the generated stories, \textit{``the generated stories are quite cohesive, I can clearly see the insights are related and under the same topics''}. He also felt comfortable with the number of facts included in the annotated graph, commenting that five to ten insights displayed in around five annotations were appropriate.
In terms of visualization, the expert was satisfied with the graph design and spoke highly of the annotation and poster style, \textit{``the combination of visualization and text helps better understand the story and it is visually appealing to read''}. 
He observed that \textit{``it's interesting to identify the order in the ranking on the nodes''}. 
Regarding the prototype system, the expert acknowledged that the interactions are user-friendly for both generating and editing data stories. In the editing phase, he found a node with a high degree based on the layout's characteristics. Then he double-clicked to obtain a list of recommended data facts, \textit{``the fact recommendation mechanism is really helpful; otherwise, I would not know what potentially interesting facts can be created. Automatic insight extraction assisted with the editor offers more flexibility for story creation''}.

% In comparing \name to traditional tools, he pointed that \textit{``the system is data-driven, the position and the size of nodes and annotations are all adaptive. Compared to design tools, this greatly reduces the design iteration time.''}. 
% % When designers design graph visualization prototypes, it is time-consuming and error-prone to associate data with the size and position of elements
% He agreed that the narrative feature is undoubtedly a significant advantage of this system compared to the general network analysis tool.

% 1. The stories generated are very cohensive, I can clearly see the insights are related and under the same topics
% 2. I also satisified with the number of insights displayed, i.e., 5 - 10 insights are displayed into ~5 groups, which is very informative and also not distracts me.. Especially, I like grouping multiple insights that relate with one single node into one box (e.g., Valjean), which is very elegant and easy to understand
% 3. The position of insight boxes also look good, they are positioned closely with the graph context but do not overlap with the main graph so that I can easily check both the insights and the graph itself.


---------related work---------
\section{Related Work}
%Our work builds on related work covering annotated visualization, automatic insight generation and organization, and graph visualization.

\subsection{Annotated Visualization}
The annotated visualization is one of the seven genres of narrative visualization proposed by Segel and Heer~\cite{segel2010narrative}. Annotations play an important role in various genres of visual narratives through guiding users' attention graphically and providing the data context ~\cite{kosara2013storytelling, choe2015characterizing, ren2017chartaccent}.
% In this paper, annotations are graphical overlaid information, such as graphical markers (such as arrows and trend lines) and/or text (such as data values or commentary), on top of a visualization to add contextual information regarding the data in the plot.
Ren \etal~\cite{ren2017chartaccent} propose a design space for annotated visualizations, identify the form of annotation (text, shapes, highlights, and images.) and the target type of annotation (data items, structural chart elements, coordinate spaces, and prior annotations). We exploit their design space and determine our visual encoding based on it in Section ~\ref{sec:visual}.
To create the annotations efficiently and effectively, a wide range of data-driven techniques and tools~\cite{kandogan2012just,hullman2013contextifier,bryan2016temporal,latif2021kori} have been proposed and developed for different use scenarios. Contextifier~\cite{hullman2013contextifier} targets at data visualization in news articles and implements a tool to automatically generate annotated stock line chart. They propose an annotation algorithm that involves visual salience, contextual relevance, and detection of key events in the company's history. Brian \etal~\cite{bryan2016temporal} study the annotations on the temporal layouts which enable the creation of the annotations with proper placement and interesting patterns. Instead of manual creation of annotations, Brath \etal~\cite{brath2018automated} automatically generate annotations, to ``automatically finding the most pertinent meaning in a given dataset.'' Kori \etal~\cite{latif2021kori} analyze the design space of chart–text references and propose a mixed-initiative interface that enables the synthesis of text and charts through interactive references.%Kori \etal~\cite{latif2021kori} analyze the design space of chart–text references through news articles and scientific papers. Based on the analysis, they propose a mixed-initiative interface that enables the synthesis of text and charts through interactive references.

Though the above works enable the data-driven annotation creation, the annotation generation for the graph data have been insufficiently touched. %Considering that the ability to tell stories with graph data is underestimated, Bounegru \etal~\cite{bounegru2017narrating} analyze a series of graph stories in journalism and concluded five perspectives for narrating graph stories. The five perspectives are later used as graph topics in Section \ref{sec:graphtopics}. 
Bach \etal~\cite{bach2016telling} discuss how to use the visual expressiveness and familiarity of comics to communicate changes in dynamic graphs. As a result, Datatoon~\cite{kim2019datatoon} is an interactive authoring tool that facilitates the creation of data comics with recommendations of four automatically-detected structural patterns including articulation points, cliques, hubs, and communities. To alleviate the barriers for telling graph stories, we provided a flexible and efficient generation and editing tool that automatically finds data facts both in attributes and structural and tells stories in the form of annotated visualizations.



\subsection{Automatic Insight Generation And Organization}
The past few years have witnessed the development of automatic insight generation and organization in both data mining and visualization communities~\cite{vartak_seedb_2015,demiralp2017foresight,ding2019quickinsights,lee2019avoiding}. 
Among them, a wide range of techniques have been dedicated to exploratory analysis. 
For example, Foresight~\cite{demiralp2017foresight} uses a rule-based visual analysis approach to extract and visualize insights from multi-dimensional data.
% SeeDB~\cite{vartak_seedb_2015, vartak_seedb_2014} helps users explore the dataset through recommending the discriminating views whose distributions deviate most from the distribution of the whole table.
Ding \etal~\cite{ding2019quickinsights} present QuickInsights, an automatic insight extraction system that discovers interesting patterns based on the statistical measures including significance and impact. 
We utilize a similar fact definition as QuickInsights does.
% and extend the scoring measures to the story-level. 
% Compared to the above studies, our work focuses on the communication purpose of visualization rather than the exploratory process. 
Not only generate meaningful data facts, Datashot \cite{wang2019datashot} and Calliope \cite{shi2020calliope} also automatically organize them in the form of fact sheets, etc. 
Datashot~\cite{wang2019datashot} organize the facts into related and meaningful topics.
% Meanwhile, Datashot~\cite{wang2019datashot} studies the presentation and automatic generation of fact sheets from tabular data. 
Calliope~\cite{shi2020calliope} further investigates automatically generating visual stories based on a logic-oriented Monte Carlo tree search algorithm. 
However, previous work is limited to multi-dimensional data while our work focuses on the fact generation and organization of graph data.
%Compared to the above studies, our work focuses on the fact generation and organization of graph data.


\subsection{Graph Visualization}
Graph visualization has been effective in a variety of ways and techniques~\cite{herman2000graph, nobre2019state}.
Node-link diagram and adjacency matrix are the two most common graph visualization forms. 
A series of studies compare node-link diagram and adjacency matrix~\cite{ghoniem2004comparison, ghoniem2005readability, okoe2018node}. Results have shown that both have their advantages and disadvantages, there is no absolute superior or inferior. Okoe et al.~\cite{okoe2018node} found that more people found the tasks being fun or interesting in the node-link diagram than in the adjacency matrix.
Engaging users is an important consideration when designing a narrative visualization, so we decided to start with the node-link diagram.
% yet presenting graphs is still a non-trivial task.
% From the aesthetic perspective, various criteria are proposed ~\cite{purchase2000effective, bennett2007aesthetics} in terms of graph layout, yet it is difficult to meet all of them. 
Various graph layout algorithms are designed for different aesthetic criteria~\cite{purchase2000effective, bennett2007aesthetics} and can be applied in different scenarios~\cite{huang2005layout, pohl2009comparing}.
Dwyer et al. compare the force-directed, orthogonal, circular and user-generated layout~\cite{dwyer2009comparison}, and find that the force-directed layout was welcomed by most users, but in specific tasks where subjective user adjustments can make the layout more understandable. Inspired by this, we add some constraints to the automatic layout algorithm for our specific presentation purposes.

Numerous tools~\cite{ellson2001graphviz,shannon2003cytoscape,bastian2009gephi,hansen2010analyzing} have been developed as solutions to facilitate graph visualization. 
% For instance, Graphviz~\cite{ellson2001graphviz} generates diagrams in useful formats with a brief graph description language.
For instance, Cytoscape~\cite{shannon2003cytoscape}, Gephi~\cite{bastian2009gephi}, and NodeXL~\cite{hansen2010analyzing} provide users with a wide range of functions for calculating graph metrics, adjusting visual attributes, and modifying layout algorithms. 
However, the above-mentioned tools are designed for graph analysis, which serves different purposes with presentation~\cite{kosara2013storytelling}.
Recently, GraphCoiffure \cite{spritzer2015towards} and Graphies~\cite{romat2019expressive} provide an interface for the smooth authoring of static communicative node-link diagrams.
However, all of these authoring tools only generate a single node-link diagram that shows the graph's overview without a specific presentation of the node or community information. In this paper, we aim to tell interesting data facts about the given graph from different granularity, including nodes, communities, and the graph as a whole.

% \rv{remove 2.4 merge with 2.3}
% \subsection{Annotation in Visual Storytelling}
% Annotations play an important role in various genres of visual narrative through guiding users' attention graphically and providing the data context ~\cite{segel2010narrative,kosara2013storytelling, choe2015characterizing,ren2017chartaccent}.
% Ren \etal~\cite{ren2017chartaccent} propose a design space for annotation visualizations, in which two dimensions, i.e. annotation form and annotation target type, are identified. We exploit their design space and determine our visual encoding based on it.
% To create the annotations efficiently and effectively, a wide range of data-driven techniques~\cite{kandogan2012just,hullman2013contextifier,bryan2016temporal} have been proposed for different visualizations. 
% Kandogan \etal~\cite{kandogan2012just} build a system to automatically annotate the clusters, outliers, and trends along with their semantic descriptions in point-based multi-dimensional visualizations. 
% Brian \etal~\cite{bryan2016temporal} study the annotations on the temporal layouts which enable the creation of the annotations with proper placement and interesting patterns. 
% Though the above works enable the data-driven annotation creation, the annotation generation for the graph data have been insufficiently touched.
  



%archive
% For example, SeeDB~\cite{vartak_seedb_2015, vartak_seedb_2014, parameswaran_seedb_2013} helps users explore the dataset through recommending the discriminating views whose distributions deviate most from the distribution of the whole table.
% Lee \etal~\cite{lee2019avoiding} promoted the necessarity of avoiding  drill-down fallacies in visual exploration. 
% and build VisPilot to guide analysts to those drill-down-fallacies-proof insights in a dataset according to ``3S'' design principles (Safety, Saliency and Succinctness). 
% The success of the above studies verify the usability of the insight generation techniques and interestingness measures, some of which are also applied in our work. 
% For example, 


% Kosara \etal~\cite{kosara2013storytelling} emphasized annotations' function in augmenting stories and guiding users in visual data-driven storytelling, especially in the context of live presentations.
% Choe \etal~\cite{choe2015characterizing} conclude a similar effects in live presentations and also emphasize that the text annotations are not replaceable by the synchronous explanations.
% Segel \etal~\cite{segel2010narrative} presented that
% presents a more general conclusion that, in different types of visual narratives, 
% text annotations can graphically guide a viewer's attention to regions of interest, suggest conclusions and provide data context. 
% Based on the two dimensions, they propose an anthoring tool called ChartAccent, which supports a palette of interactions for the data-driven annotation. 
% We construct our design space by adapting theirs to the graph annotations. 

% Hullman \etal~\cite{hullman2013contextifier} focus on stock line chart and present Contextifier, an automatic annotation generation system, which annotated the stock behaviors based on the news articles.

% and are a non-trivial problem due to the following reasons. 
% To start with, the placement of the annotations increase the layout difficulty in network presentation when there is less space for the network annotations. Secondly, annotations of different elements in network data i.e. community, node, need to be placed together, which can lead to visual clutters. 


%Narrative visualization is a method of visually telling data stories, which can divided into seven specific genres including annotated charts according to Segel and Heer\cite{segel2010narrative}.
% For example, ChartAccent \cite{ren2017chartaccent} allows people to generate expressive manual and data-driven annotations to enhance charts.
% In addition, Datashot \cite{wang2019datashot} and Calliope \cite{shi2020calliope} automatically generate meaningful data facts and narrate the story in the form of fact Sheets, etc. 

%Narrative Visualization - Network Narratives
%“Narrating Networks” Narrative functions of networks in journalism

----------------------

==> tables/annotationTemplates.tex <==
\begin{table*}[bp]
\renewcommand\arraystretch{1.3}
\linespread{1.5}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\centering
\caption{Text Annotation Templates}
\begin{tabular}{|p{0.10 \textwidth}|p{0.3 \textwidth}|p{0.52 \textwidth}|}
\toprule
\textbf{Type}         & \textbf{Template}      & \textbf{Example}                    \\ \hline
Extreme      & \textless{}Focus\textgreater\space is a \textless{}Measure Translation\textgreater\space \textless{}Partition\textgreater\space based on \textless{}Measure\textgreater\space   in \textless{}Subspace\textgreater{}                                           & \textless{}Valjean\textgreater\space is an \textless{}influential\textgreater\space \textless{}node\textgreater\space based on \textless{}degree\textgreater\space in \textless{}\img{pictures/inline/community1}\textgreater{}\space.  \\ \hline
Rank         & \textless{}Focus\textgreater\space are top-3 \textless{}Measure Translation\textgreater\space  \textless{}Partition\textgreater\space based on \textless{}Measure\textgreater\space in \textless{}Subspace\textgreater{} & \textless{} \img{pictures/inline/community1}, \img{pictures/inline/community3} and \img{pictures/inline/community2}\textgreater\space are top-3 \textless{}cohesive\textgreater\space \textless{}communities\textgreater\space based on \textless{}density\textgreater{}\space.  \\ \hline
Outlier      & \textless{}Focus\textgreater\space is an outlier based on \textless{}Measure\textgreater\space in \textless{}Subspace\textgreater{} & \textless{}Hedwig\textgreater\space is an outlier based on \textless{}degree\textgreater\space in \textless{}\img{pictures/inline/community1}\textgreater{}.\\ \hline
Proportion   & \textless{}Focus\textgreater\space occupies \textless{}Derived Value\textgreater\space \textless{}Measure\textgreater\space in \textless{}Subspace\textgreater{}     & \textless{}Harry Potter\textgreater\space occupies \textless{}23.4\%\textgreater\space \textless{}degree\textgreater\space in \textless{}\img{pictures/inline/community1}\textgreater{} \space.\\ \hline
Distribution & Distribution of \textless{}Partition\textgreater\space \textless{}Measure\textgreater\space in \textless{}Subspace\textgreater{}        & Distribution of \textless{}nodes'\textgreater\space  \textless{}eigenvector centrality\textgreater\space  in \textless{}\img{pictures/inline/community1}\textgreater{}\space.  \\ \hline
Evenness     & The \textless{}Partition\textgreater\space have a even distribution based on the values of \textless{}Measure\textgreater{}                                                                           & The \textless{}nodes\textgreater\space  have a even distribution based on the values of \textless{}degree\textgreater{}\space.  \\ \bottomrule
\end{tabular}
\label{tab:templates}
\end{table*}


==> tables/description.tex <==
\begin{table*}[bp]
\renewcommand\arraystretch{1.3}
\linespread{1.5}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\centering
\caption{Descriptions Of Technical Terms}
\begin{tabular}{|p{0.22 \textwidth}|p{0.22 \textwidth}|p{0.4 \textwidth}|}
\toprule
\textbf{Measure}         & \textbf{Description}      & \textbf{Example}                    \\ \hline
Degree      & Super connector                    &  Node A is a super connector as it has the most connections.
\\ \hline
PageRank score         & 
Important
& 
Node A is an important node because it has 
has many connections and important neighbors.
\\ \hline
Eigenvector centrality   & 
Influential
& 
Node A is an influential node while considering 
both direct and indirect connections.
\\ \hline
Inside edge number   & 
Close internal relationship
& 
Community A has a close internal relationship based on the highest inside connections.
\\ \hline

Average degree/ Density 
& 
Highly connected 
& 
Community A is a highly connected community based on frequent internal connections.			
			
\\ \hline
Average out degree fraction/Maximum out degree fraction
& 
Strong external connectivity
& 
Community A has strong external connectivity based on frequent external connections.				
				
\\ \hline
Separability
& 
Isolated
& 
Community A is an isolated community based on scarce external connections.	
\\ \bottomrule
\end{tabular}
\label{tab:description}
\end{table*}

==> tables/factType-new.tex <==
% \newcommand{focuscolor}{blue}
% \newcommand{mtcolor}{green}
% \newcommand{partitioncolor}{purple}
% \newcommand{measurecolor}{yellow}
% \newcommand{subspacecolor}{red}
% \newcommand{dvcolor}{violet}
\definecolor{mtcolor}{RGB}{223, 159, 157}
\definecolor{subspacecolor}{RGB}{107, 148, 104}
\definecolor{measurecolor}{RGB}{174, 133, 175}
\definecolor{dvcolor}{RGB}{214, 126, 58}
\definecolor{partitioncolor}{RGB}{182, 53, 43}
\definecolor{focuscolor}{RGB}{54, 108, 157}

\begin{table*}[bp]
\renewcommand\arraystretch{1.3}
\linespread{1.5}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\centering
\caption{Fact Overview. In the table, \textcolor{focuscolor}{F} refers to the focus components, e.g. Valjean. \textcolor{mtcolor}{D} refers to measure description. \textcolor{partitioncolor}{P} refers to the partition. \textcolor{measurecolor}{M} refers to the measure.  \textcolor{subspacecolor}{S} refers to the subspace. \textcolor{dvcolor}{V} refers to the derived value.}
\begin{tabular}{|p{0.10 \textwidth}|p{0.25 \textwidth}|p{0.15 \textwidth}|p{0.40 \textwidth}|}
\toprule
\textbf{Type}  &Description  & \textbf{Template}      & \textbf{Scoring Function}                    \\ \hline
Extreme    &Extreme facts refer to the corresponding community/node of the maximum feature value    & \textcolor{focuscolor}{\textless{}F\textgreater}\space is a \textcolor{mtcolor}{\textless{}D\textgreater}\space \textcolor{partitioncolor}{\textless{}P\textgreater}\space based on \textcolor{measurecolor}{\textless{}M\textgreater}\space   in \textcolor{subspacecolor}{\textless{}S\textgreater}{}                                           &
\begin{enumerate*}
    \item Extracting the feature vector of all nodes/communities.
    \item Calculating the interestness based on the method used in \cite{shi2020calliope}
\end{enumerate*}

% Remove the maximum value $x_{max}$ and then predict the maximum value $\tilde{x}_{\texttt{max}}$ based on the residual distribution. The interestness score is defined as $1-p$ where p is the $p-value$ of the hypothesis that $\tilde{x}_{\texttt{max}}=x_{max}$
  \\ \hline
Rank    &Rank facts share a similar notion with the extreme while Rank facts focus on top-k (3 in our case) nodes/communities. & \textcolor{focuscolor}{\textless{}F\textgreater}\space are top-3 \textcolor{mtcolor}{\textless{}D\textgreater}\space  \textcolor{partitioncolor}{\textless{}P\textgreater}\space based on \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{} & 
\begin{enumerate*}
    \item Extracting the feature vector of all nodes/communities.
    \item Calculating the interestness score based on the method used in \cite{shi2020calliope}
\end{enumerate*} \\
% Infer a Gaussian distribution $D$ based on the residuals of power law regression. Predict the largest value   $\hat{x}_{max}$ with the residual $R$. Define the interestness score as $1-p$ \\ 
\hline
Outlier    &The Outlier fact type measures how a node deviates from its neighborhood and the whole graph.    & \textcolor{focuscolor}{\textless{}F\textgreater}\space is an outlier based on \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{} &  
\begin{enumerate*}
    \item Calculating the neighborhood's average score $\tilde{x}_i$ of each node $i$.
    \item Defining node $i$'s interestness score as $\frac{|\tilde{x}_i-x_i|}{\max(\tilde{x}_i,x_i)}$.
\end{enumerate*}

\\ \hline
Proportion  &Proportion measure the extent to which the leading value dominates the feature entries.   & \textcolor{focuscolor}{\textless{}F\textgreater}\space occupies \textcolor{dvcolor}{\textless{}V\textgreater}\space \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{}     & 
\begin{enumerate*}
    \item Sorting the feature vector in descending order to obtain the maximum value $x_{max}$.
    \item Defining interestness score as $\min{(1, \frac{2\times x_{\texttt{max}}}{\sum x})}$
\end{enumerate*}
 \\ \hline
Distribution  & The distribution fact type is to determine if the feature vector are well-modeled by a Gaussian distribution & Distribution of \textcolor{partitioncolor}{\textless{}P\textgreater}\space \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{}        & \begin{enumerate*}
    \item Performing Shapiro–Wilk test on the given feature vector to obtain the $p$-value.
    \item Defining interestness as $1-p$.
\end{enumerate*} \\ \hline
Evenness    &Evenness determines if the entries from the feature vector are uniformly distributed.  & The \textcolor{partitioncolor}{\textless{}P\textgreater}\space have a even distribution based on the values of \textcolor{measurecolor}{\textless{}M\textgreater}{}                                                                       & 
\begin{enumerate*}
    \item Perform the Chi-squared test against the null hypothesis that the feature vector should be the a constant vector, to obtain the $p$-value.
    \item Defining interestness as $1-p$.
\end{enumerate*}
  \\ \bottomrule
\end{tabular}
\label{tab:fact-overview}
\end{table*}

% % \newcommand{focuscolor}{blue}
% % \newcommand{mtcolor}{green}
% % \newcommand{partitioncolor}{purple}
% % \newcommand{measurecolor}{yellow}
% % \newcommand{subspacecolor}{red}
% % \newcommand{dvcolor}{violet}
% \definecolor{mtcolor}{RGB}{223, 159, 157}
% \definecolor{subspacecolor}{RGB}{107, 148, 104}
% \definecolor{measurecolor}{RGB}{174, 133, 175}
% \definecolor{dvcolor}{RGB}{214, 126, 58}
% \definecolor{partitioncolor}{RGB}{182, 53, 43}
% \definecolor{focuscolor}{RGB}{54, 108, 157}

% \begin{table*}[bp]
% \renewcommand\arraystretch{1.3}
% \linespread{1.5}
% \setlength\aboverulesep{0pt}
% \setlength\belowrulesep{0pt}
% \centering
% \caption{Fact Overview. In the table, \textcolor{focuscolor}{F} refers to the focus components, e.g. Valjean. \textcolor{mtcolor}{MT} refers to measure translation. \textcolor{partitioncolor}{P} refers to the partition. \textcolor{measurecolor}{M} refers to the measure. \textcolor{subspacecolor}{S} refers to the subspace.}
% \begin{tabular}{|p{0.10 \textwidth}|p{0.30 \textwidth}|p{0.25 \textwidth}|p{0.25 \textwidth}|}
% \toprule
% \textbf{Type}  &Description  & \textbf{Template}      & \textbf{Example}                    \\ \hline
% Extreme    &Extreme insight refers to the corresponding community/node of the maximum feature value    & \textcolor{focuscolor}{\textless{}F\textgreater}\space is a \textcolor{mtcolor}{\textless{}MT\textgreater}\space \textcolor{partitioncolor}{\textless{}P\textgreater}\space based on \textcolor{measurecolor}{\textless{}M\textgreater}\space   in \textcolor{subspacecolor}{\textless{}S\textgreater}{}                                           & \textcolor{focuscolor}{Valjean}\space is an \textcolor{mtcolor}{influential}\space \textless{}node\textgreater\space based on \textcolor{measurecolor}{degree}\space in \textless{}\img{pictures/inline/community1}\textgreater{}\space.  \\ \hline
% Rank    &Rank facts share a similar notion with the extreme while Rank facts focus on top-k (3 in our case) nodes/communities. & \textcolor{focuscolor}{\textless{}F\textgreater}\space are top-3 \textcolor{mtcolor}{\textless{}MT\textgreater}\space  \textcolor{partitioncolor}{\textless{}P\textgreater}\space based on \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{} & \textless{} \img{pictures/inline/community1}, \img{pictures/inline/community3} and \img{pictures/inline/community2}\textgreater\space are top-3 \textcolor{mtcolor}{cohesive communities}\space based on \textless{}density\textgreater{}\space.  \\ \hline
% Outlier    &The Outlier fact type measures how a node deviates from its neighborhood and the whole graph.    & \textcolor{focuscolor}{\textless{}F\textgreater}\space is an outlier based on \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{} & \textcolor{focuscolor}{Hedwig}\space is an outlier based on \textcolor{measurecolor}{degree}\space in \textless{}\img{pictures/inline/community1}\textgreater{}.\\ \hline
% Proportion  &Proportion measure the extent to which the leading value dominates the feature entries.   & \textcolor{focuscolor}{\textless{}F\textgreater}\space occupies \textcolor{dvcolor}{\textless{}DV\textgreater}\space \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{}     & \textcolor{focuscolor}{Harry Potter}\space occupies \textcolor{dvcolor}{23.4\%}\space \textcolor{measurecolor}{degree}\space in \textless{}\img{pictures/inline/community1}\textgreater{} \space.\\ \hline
% Distribution  & The distribution fact type is to determine if entries of the feature vector are well-modeled by a Gaussian distribution & Distribution of \textcolor{partitioncolor}{\textless{}P\textgreater}\space \textcolor{measurecolor}{\textless{}M\textgreater}\space in \textcolor{subspacecolor}{\textless{}S\textgreater}{}        & Distribution of \textcolor{focuscolor}{nodes'}\space  \textcolor{measurecolor}{eigenvector centrality}\space  in \textless{}\img{pictures/inline/community1}\textgreater{}\space.  \\ \hline
% Evenness    &Evenness determines if the entries from the feature vector are uniformly distributed.  & The \textcolor{partitioncolor}{\textless{}P\textgreater}\space have a even distribution based on the values of \textcolor{measurecolor}{\textless{}M\textgreater}{}                                                                           & The \textcolor{focuscolor}{nodes}\space  have a even distribution based on the values of \textcolor{measurecolor}{degree}{}\space.  \\ \bottomrule
% \end{tabular}
% \label{tab:fact-overview}
% \end{table*}


==> tables/measureTranslation.tex <==
\begin{table*}[bp]
\renewcommand\arraystretch{1.3}
\linespread{1.5}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\centering
\caption{Measure Translation}
\begin{tabular}{|p{0.12 \textwidth}|p{0.14 \textwidth}|p{0.16 \textwidth}|p{0.44 \textwidth}|}

\toprule
\textbf{Partition Level} & \textbf{Measure}                          & \textbf{Description}           & \textbf{Example}                                                                       \\ \hline
Node      & Degree                           & Influential           & Valjean is an influential node based on degree.                               \\ \hline
Node      & Eigenvector centrality           & Influential           & Gavoroche is an influential node based on eigenvector centrality.              \\ \hline
Node      & PageRank score                   & Influential           & Harry Potter is an influential node based on PageRank score.                  \\ \hline
Community & Size                            & Influential           & \img{pictures/inline/community1} is an influential community based on size.                                 \\ \hline
Community & Inside edge number               & Cohesive              & \img{pictures/inline/community1} is a cohesive community based on inside edge number.                   \\ \hline
Community & Density                          & Cohesive              & \img{pictures/inline/community1} is a cohesive community based on density.                              \\ \hline
Community & Average degree                   & Cohesive              & \img{pictures/inline/community1} is a cohesive community based on average degree.                       \\ \hline
Community & Triangle participation ratio (TPR)     & Cohesive              & \img{pictures/inline/community1} is a cohesive community based on triangle participation ratio.         \\ \hline
Community & Average-out degree fraction & External Connectivity & \img{pictures/inline/community1} enjoys a great connectivity based on average out degree fraction. \\ \hline
Community & Maximum-out degree fraction & External Connectivity & \img{pictures/inline/community1} enjoys a great connectivity based on maximum out degree fraction. \\ \hline
Community & Separability & Well Separated  & \img{pictures/inline/community1} is well separated from the rest of the network based on separability.  \\ \hline
Community & Cut Ratio & Well Separated  & \img{pictures/inline/community1} is well separated from the rest of the network based on cut ratio. \\ \bottomrule
\end{tabular}
\vspace{1mm}
\label{tab:measure_translation}
\end{table*}


==> tables/phraseGeneralization.tex <==
\begin{table}[H]
\centering
\caption{Conjunction Generalization}
\renewcommand\arraystretch{1.3}
\linespread{1.5}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\begin{tabular}{ l l }
\toprule
\textbf{Narrative Relation} & \textbf{Conjunction}       \\ \hline
Similarity         & Similarly   \\ \hline
Contrast           & By contrast  \\ \hline
Elaboration        & To elaborate \\ \hline
Generalization     & Generally    \\ \bottomrule
\end{tabular}
\label{tab:phrase_generalization}
\end{table}
